Phase diagram of UPt$_3$ in the $E_{1g}$ model

The phase diagram of the unconventional superconductor UPt$_3$ is explained under the long-standing hypothesis that the pair wavefunction belongs to the $E_{1g}$ representation of the point group. The main objection to this theory has been that it disagrees with the experimental phase diagram when a field is applied along the c-axis. By a careful analysis of the free energy this objection is shown to be incorrect. This singlet theory also explains the unusual anisotropy in the upper critical field curves, often thought to indicate a triplet pair function.

==> crossing <==
%!PS-Adobe-3.0
%%Creator: Windows PSCRIPT
%%Title: CROSSING.AI
%%BoundingBox: 18 9 593 784
%%DocumentNeededResources: (atend)
%%DocumentSuppliedResources: (atend)
%%Pages: (atend)
%%BeginResource: procset Win35Dict 3 1
/Win35Dict 60 dict def Win35Dict begin/bd{bind def}bind def/in{72
mul}bd/ed{exch def}bd/ld{load def}bd/tr/translate ld/gs/gsave ld/gr
/grestore ld/fPP false def/SS{fPP{/SV save def}{gs}ifelse}bd/RS{fPP{SV
restore}{gr}ifelse}bd/EJ{gsave showpage grestore}bd/#C{userdict begin
/#copies ed end}bd/FEbuf 2 string def/FEglyph(G  )def/FE{1 exch{dup
16 FEbuf cvrs FEglyph exch 1 exch putinterval 1 index exch FEglyph
cvn put}for}bd/SM{/iRes ed/cyP ed/cxPg ed/cyM ed/cxM ed 0 ne{0 cyP
72 mul 100 div tr -90 rotate}if pop}bd/CB{moveto/dy ed/dx ed dx 0 rlineto
0 dy rlineto dx neg 0 rlineto closepath clip newpath}bd/ErrHandler{errordict
dup maxlength exch length gt dup{errordict begin}if/errhelpdict 12
dict def errhelpdict begin/stackunderflow(operand stack underflow)def
/undefined(this name is not defined in a dictionary)def/VMerror(you have used up all the printer's memory)def
/typecheck(operator was expecting a different type of operand)def
/ioerror(input/output error occured)def end{end}if errordict begin
/handleerror{$error begin newerror{/newerror false def showpage 72
72 scale/x .25 def/y 9.6 def/Helvetica findfont .2 scalefont setfont
x y moveto(Offending Command = )show/command load{dup type/stringtype
ne{(max err string)cvs}if show}exec/y y .2 sub def x y moveto(Error = )show
errorname{dup type dup( max err string )cvs show( : )show/stringtype
ne{( max err string )cvs}if show}exec errordict begin errhelpdict errorname
known{x 1 add y .2 sub moveto errhelpdict errorname get show}if end
/y y .4 sub def x y moveto(Stack =)show ostack{/y y .2 sub def x 1
add y moveto dup type/stringtype ne{( max err string )cvs}if show}forall
showpage}if end}def end}bd end
%%EndResource
/SVDoc save def
%%EndProlog
%%BeginSetup
Win35Dict begin
ErrHandler
statusdict begin 0 setjobtimeout end
statusdict begin statusdict /jobname (CROSSING.AI) put end
/oldDictCnt countdictstack def {}stopped 
{ countdictstack oldDictCnt lt { Win35Dict begin } 
{1 1 countdictstack oldDictCnt sub {pop end } for } ifelse } if 
/oldDictCnt countdictstack def {letter
}stopped 
{ countdictstack oldDictCnt lt { Win35Dict begin } 
{1 1 countdictstack oldDictCnt sub {pop end } for } ifelse } if 
[
{mark 1.0 1.0 .98 .9 .82 .68 .56 .48 .28 .1 .06 .0 counttomark dup 3 add -1 roll exch 2 sub mul dup floor cvi dup 3 1 roll sub exch dup  3 add index exch 2 add index dup 4 1 roll sub mul add counttomark 1 add 1 roll  cleartomark } bind
/exec load currenttransfer /exec load] cvx settransfer
%%EndSetup
%%Page: 1 1
%%PageResources: (atend)
SS
0 0 25 11 798 1100 300 SM
2394 3231 0 0 CB
%%BeginDocument: Adobe Illustrator(TM) for Windows, version
%!PS-Adobe-3.0 EPSF-3.0
%%Creator: Adobe Illustrator(TM) for Windows, version 4.0
%%For: (Robert J. Joynt                         ) (Physics Dept.  UW - Madison             )
%%CreationDate: (11/30/94) (5:20 PM)
%%BoundingBox: 46 39 547 710
%%DocumentProcessColors: Black
%%DocumentFonts: Times-Roman
%%+ Times-Italic
%%+ Times-BoldItalic
%%DocumentSuppliedResources: procset Adobe_packedarray 2.0 0
%%+ procset Adobe_cmykcolor 1.1 0
%%+ procset Adobe_cshow 1.1 0
%%+ procset Adobe_customcolor 1.0 0
%%+ procset Adobe_typography_AI3 1.0 0
%%+ procset Adobe_IllustratorA_AI3 1.0 0
%AI3_ColorUsage: Black&White
%AI3_TemplateBox: 300 225 300 225
%AI3_TileBox: 0 0 575 775
%AI3_DocumentPreview: Header
%%Template:
%%PageOrigin:0 0
%%AI3_PaperRect:-18 784 594 -8
%%AI3_Margin:18 -9 -19 8
%%EndComments
%%BeginProlog
%%BeginResource: procset Adobe_packedarray 2.0 0
%%Title: (Packed Array Operators)
%%Version: 2.0 
%%CreationDate: (8/2/90) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

userdict /Adobe_packedarray 5 dict dup begin put
/initialize			% - initialize -
{
/packedarray where
	{
	pop
	}
	{
	Adobe_packedarray begin
	Adobe_packedarray
		{
		dup xcheck
			{
			bind
			} if
		userdict 3 1 roll put
		} forall
	end
	} ifelse
} def
/terminate			% - terminate -
{
} def
/packedarray		% arguments count packedarray array
{
array astore readonly
} def
/setpacking			% boolean setpacking -
{
pop
} def
/currentpacking		% - setpacking boolean
{
false
} def
currentdict readonly pop end
%%EndResource
Adobe_packedarray /initialize get exec
%%BeginResource: procset Adobe_cmykcolor 1.1 0
%%Title: (CMYK Color Operators)
%%Version: 1.1 
%%CreationDate: (1/23/89) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

currentpacking true setpacking
userdict /Adobe_cmykcolor 4 dict dup begin put
/initialize			% - initialize -
{
/setcmykcolor where
	{
	pop
	}
	{
	userdict /Adobe_cmykcolor_vars 2 dict dup begin put
	/_setrgbcolor
		/setrgbcolor load def
	/_currentrgbcolor
		/currentrgbcolor load def
	Adobe_cmykcolor begin
	Adobe_cmykcolor
		{
		dup xcheck
			{
			bind
			} if
		pop pop
		} forall
	end
	end
	Adobe_cmykcolor begin
	} ifelse
} def
/terminate			% - terminate -
{
currentdict Adobe_cmykcolor eq
	{
	end
	} if
} def
/setcmykcolor		% cyan magenta yellow black setcmykcolor -
{
1 sub 4 1 roll
3
	{
	3 index add neg dup 0 lt
		{
		pop 0
		} if
	3 1 roll
	} repeat
Adobe_cmykcolor_vars /_setrgbcolor get exec
pop
} def 
/currentcmykcolor	% - currentcmykcolor cyan magenta yellow black
{
Adobe_cmykcolor_vars /_currentrgbcolor get exec
3
	{
	1 sub neg 3 1 roll
	} repeat
0
} def
currentdict readonly pop end
setpacking

%%EndResource
%%BeginResource: procset Adobe_cshow 1.1 0
%%Title: (cshow Operator)
%%Version: 1.1 
%%CreationDate: (1/23/89) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

currentpacking true setpacking
userdict /Adobe_cshow 3 dict dup begin put
/initialize			% - initialize -
{
/cshow where
	{
	pop
	}
	{
	userdict /Adobe_cshow_vars 1 dict dup begin put
	/_cshow		% - _cshow proc
		{} def
	Adobe_cshow begin
	Adobe_cshow
		{
		dup xcheck
			{
			bind
			} if
		userdict 3 1 roll put
		} forall
	end
	end
	} ifelse
} def
/terminate			% - terminate -
{
} def
/cshow				% proc string cshow -
{
exch
Adobe_cshow_vars
	exch /_cshow
	exch put
	{
	0 0 Adobe_cshow_vars /_cshow get exec
	} forall
} def
currentdict readonly pop end
setpacking

%%EndResource
%%BeginResource: procset Adobe_customcolor 1.0 0
%%Title: (Custom Color Operators)
%%Version: 1.0 
%%CreationDate: (5/9/88) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

currentpacking true setpacking
userdict /Adobe_customcolor 5 dict dup begin put
/initialize			% - initialize -
{
/setcustomcolor where
	{
	pop
	}
	{
	Adobe_customcolor begin
	Adobe_customcolor
		{
		dup xcheck
			{
			bind
			} if
		pop pop
		} forall
	end
	Adobe_customcolor begin
	} ifelse
} def
/terminate			% - terminate -
{
currentdict Adobe_customcolor eq
	{
	end
	} if
} def
/findcmykcustomcolor	% cyan magenta yellow black name findcmykcustomcolor object
{
5 packedarray
}  def
/setcustomcolor		% object tint setcustomcolor -
{
exch
aload pop pop
4
	{
	4 index mul 4 1 roll
	} repeat
5 -1 roll pop
setcmykcolor
} def
/setoverprint		% boolean setoverprint -
{
pop
} def
currentdict readonly pop end
setpacking

%%EndResource
%%BeginResource: procset Adobe_typography_AI3 1.0 0
%%Title: (Typography Operators)
%%Version: 1.0 
%%CreationDate:(5/31/90) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

currentpacking true setpacking
userdict /Adobe_typography_AI3 46 dict dup begin put
/initialize			% - initialize -
{
/TZ
 where
	{
	pop
	}
	{
	Adobe_typography_AI3 begin
	Adobe_typography_AI3
		{
		dup xcheck
			{
			bind
			} if
		pop pop
		} forall
	end
	Adobe_typography_AI3 begin
	} ifelse
} def
/terminate			% - terminate -
{
currentdict Adobe_typography_AI3 eq
	{
	end
	} if
} def

% [ number value stream [ array for encoding modification ] modifyEncoding ==> [ modified array ]
/modifyEncoding
{
	/_tempEncode exch ddef
	
	% pointer for sequential encodings
	/_pntr 0 ddef
	
	{
		% get bottom object
		counttomark -1 roll

		% is it a mark ?
		dup type dup /marktype eq 		
		{
			% exit
			pop pop exit
		}
		{
			% ... object ... type ....

			% insert if a nametype
			/nametype eq
			{
				% insert the name at _pntr and increment pointer
				_tempEncode /_pntr dup load dup 3 1 roll 1 add ddef 3 -1 roll
				put
			}
			{
				% reset _pntr if it's a number
				/_pntr exch ddef					
			}
			ifelse
		}
		ifelse
	}
	loop	
	
	% return the modified encoding
	_tempEncode
}
def

/TE	% Set std platform encoding 	% (encoding pairs) TE -
{
	StandardEncoding 256 array copy modifyEncoding 
	/_nativeEncoding exch def
} def

% re-define font
% expected arguments
% for 'normal fonts : 
%	[ /_Helvetica-Bold/Helvetica-Bold direction fontScript defaultEncoding TZ
%
% for cartographic, pictographic, and expert fonts :
% 	[ ... number value stream ... /_Helvetica-Bold/Helvetica-Bold 
%	direction fontScript defaultEncoding TZ
/TZ		
{
	% platform dependent coding flag
	/_useNativeEncoding exch def

	% pop fontScript & direction
	pop pop
	
	% create a new dictionary with length
	% equal to original dictionary length + 2
	% copy all the key/value pairs except FID
	findfont dup length 2 add dict
	
	begin
	
		% copy all the values but the FID
		% into the new dictionary
		mark exch
		{
			1 index /FID ne { def } if cleartomark mark
		}
		forall
		% discard last mark
		pop
		
		% define FontName
		/FontName exch def
		
		% if no re-encoding stream is present
		% then if the base encoding vector of the font
		% is the same as StandardEncoding
		% and the use platform encoding flag is true
		% then install AI platform encoding
		% else leave the base encoding in effect

		counttomark 0 eq
		{
			Encoding StandardEncoding eq 1 _useNativeEncoding eq and
			{
				/Encoding _nativeEncoding def
			}
			if
			% clean up
			cleartomark
		}
		{	
			% custom encoding to be done
			% start off with a copy of the font's standard encoding
			/Encoding load 256 array copy 
			modifyEncoding /Encoding exch def
		}
		ifelse		
		FontName currentdict
	end
	
	% register the new font
	definefont pop
}
def

% text painting operators
/tr					% string tr ax ay string 
{
_ax _ay 3 2 roll
} def
/trj				% string trj cx cy fillchar ax ay string 
{
_cx _cy _sp _ax _ay 6 5 roll
} def

/a0
{
/Tx	% text							% textString Tx -
	{
	dup 
	currentpoint 3 2 roll
	tr _psf
	newpath moveto
	tr _ctm _pss
	} ddef
/Tj	% justified text				% textString Tj -
	{
	dup
	currentpoint 3 2 roll
	trj _pjsf
	newpath moveto
	trj _ctm _pjss
	} ddef
	
} def
/a1
{
W B
} def

/e0
{
/Tx	% text							% textString Tx -
	{
	tr _psf
	} ddef
/Tj	% justified text				% textString Tj -
	{
	trj _pjsf
	} ddef
} def

/e1
{
W F 
} def


/i0
{
/Tx	% text							% textString Tx -
	{
	tr sp
	} ddef
/Tj	% justified text				% textString Tj -
	{
	trj jsp
	} ddef
} def

/o0
{
/Tx	% text							% textString Tx -
	{
	tr sw rmoveto
	} ddef
/Tj	% justified text				% textString Tj -
	{
	trj swj rmoveto
	} ddef
} def

/r0
{
/Tx	% text							% textString Tx -
	{
	tr _ctm _pss
	} ddef
/Tj	% justified text				% textString Tj -
	{
	trj _ctm _pjss
	} ddef
} def
/r1
{
W S
} def

% font operators

% Binding
/To	% begin text 					% bindType To -
{
	pop _ctm currentmatrix pop
} def

/TO	% end text					% TO -
{
	Te _ctm setmatrix newpath
} def

% Text paths
/Tp	% begin text path				% a b c d tx ty startPt Tp -
{
	pop _tm astore pop _ctm setmatrix 
	2 dict begin /W {} def /h {} def
} def

/TP	% end text path					% TP -
{
	end
	iTm 0 0 moveto
} def

% Render mode & matrix operators
/Tr	% begin render					% render Tr - 
{
	Te currentpoint newpath moveto
	dup 8 eq {pop 0} {dup 9 eq {pop 1} if} ifelse
	dup /_render exch ddef
	_renderStart exch get load exec
} def

/iTm % internal set text matrix		% - iTm -	(uses _tm as implicit argument)
{
_ctm setmatrix _tm concat 0 _rise translate _hs 1 scale
} def

/Tm % set text matrix				% a b c d tx ty Tm -
{
_tm astore pop iTm 0 0 moveto
} def

/Td % translate text matrix 		% tx ty Td -
{
_mtx translate _tm _tm concatmatrix pop iTm 0 0 moveto
} def

/Te	% end render					% - Te -
{
	_render -1 eq {} {_renderEnd _render get dup null ne {load exec} {pop} ifelse} ifelse
	/_render -1 ddef
} def


% Attributes
/Ta	% set alignment					% alignment Ta -
{
pop
} def

/Tf	% set font name and size		% fontname size Tf -
{
dup 1000 div /_fScl exch ddef
exch findfont exch scalefont setfont
} def

/Tl	% set leading					% leading paragraphLeading Tl -
{
pop
0 exch _leading astore pop
} def

/Tt	% set user tracking				% userTracking Tt -
{
pop
} def

/TW % set word spacing				% minSpace optSpace maxSpace TW -
{
3 npop
} def

/Tw	% set computed word spacing		% wordSpace Tw
{
/_cx exch ddef
} def

/TC % set character spacing			% minSpace optSpace maxSpace TC -
{
3 npop
} def

/Tc	% set computed char spacing 	% charSpace Tc -
{
/_ax exch ddef
} def

/Ts % set super/subscripting (rise)	% rise Ts -
{
/_rise exch ddef
currentpoint
iTm
moveto
} def

/Ti	% set indentation				% firstStartIndent otherStartIndent stopIndent Ti -
{
3 npop
} def

/Tz % set horizontal scaling		% scalePercent Tz -
{
100 div /_hs exch ddef
iTm
} def

/TA % set pairwise kerning			% autoKern TA -
									%	autoKern = 0 -> no pair kerning
									%			 = 1 -> automatic pair kerning
{
pop
} def

/Tq % set hanging quotes			% hangingQuotes Tq -
									%	hangingQuotes 	= 0 -> no hanging quotes
									%			 		= 1 -> hanging quotes
{
pop
} def


% Text Bodies
/TX {pop} def

%/Tx	% non-justified text			% textString Tx -
%/Tj	% justified text				% textString Tj -

/Tk	% kern							% autoKern kernValue Tk -
									%  	autoKern = 0 -> manual kern, = 1 -> auto kern
									%	kernValue = kern value in em/1000 space
{
exch pop _fScl mul neg 0 rmoveto
} def
/TK	% non-printing kern				% autoKern kernValue TK -
{
2 npop
} def

/T* % carriage return & line feed	% - T* -
{
_leading aload pop neg Td
} def

/T*- % carriage return & negative line feed	% - T*- -
{
_leading aload pop Td
} def

/T-	% print a discretionary hyphen	% - T- -
{
_hyphen Tx
} def

/T+	% discretionary hyphen hyphen	% - T+ -
{} def

/TR	% reset pattern matrix 			% a b c d tx ty TR -
{
_ctm currentmatrix pop 	
_tm astore pop 
iTm 0 0 moveto 
} def

/TS	% special chars					% textString justified TS -
{
0 eq {Tx} {Tj} ifelse
} def

currentdict readonly pop end
setpacking

%%EndResource
%%BeginResource: procset Adobe_IllustratorA_AI3 1.0 0
%%Title: (Adobe Illustrator (R) Version 3.0 Abbreviated Prolog)
%%Version: 1.0 
%%CreationDate: (7/22/89) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

currentpacking true setpacking
userdict /Adobe_IllustratorA_AI3 61 dict dup begin put
% initialization
/initialize				% - initialize -
{
userdict /Adobe_IllustratorA_AI3_vars 46 dict dup begin put

% paint operands
/_lp /none def
/_pf {} def
/_ps {} def
/_psf {} def
/_pss {} def
/_pjsf {} def
/_pjss {} def
/_pola 0 def
/_doClip 0 def

% paint operators
/cf	currentflat def	% - cf flatness

% typography operands
/_tm matrix def
/_renderStart [/e0 /r0 /a0 /o0 /i0 /i0 /i0 /i0] def 
/_renderEnd [null null null null /e1 /r1 /a1 /clip] def
/_render -1 def
/_rise 0 def
/_ax 0 def			% x character spacing	(_ax, _ay, _cx, _cy follows awidthshow naming convention)
/_ay 0 def			% y character spacing
/_cx 0 def			% x word spacing
/_cy 0 def			% y word spacing
/_leading [0 0] def
/_ctm matrix def
/_mtx matrix def
/_sp 16#020 def
/_hyphen (-) def
/_fScl 0 def
/_cnt 0 def
/_hs 1 def
/_nativeEncoding 0 def
/_useNativeEncoding 0 def
/_tempEncode 0 def
/_pntr 0 def

% typography operators
/Tx {} def
/Tj {} def

% compound path operators
/CRender {} def

% printing
/_AI3_savepage {} def

% color operands
/_gf null def
/_cf 4 array def
/_if null def
/_of false def
/_fc {} def
/_gs null def
/_cs 4 array def
/_is null def
/_os false def
/_sc {} def
/_i null def
Adobe_IllustratorA_AI3 begin
Adobe_IllustratorA_AI3
	{
	dup xcheck
		{
		bind
		} if
	pop pop
	} forall
end
end
Adobe_IllustratorA_AI3 begin
Adobe_IllustratorA_AI3_vars begin
newpath
} def
/terminate				% - terminate -
{
end
end
} def
% definition operators
/_					% - _ null
null def
/ddef				% key value ddef -
{
Adobe_IllustratorA_AI3_vars 3 1 roll put
} def
/xput				% key value literal xput -
{
dup load dup length exch maxlength eq
	{
	dup dup load dup
	length 2 mul dict copy def
	} if
load begin def end
} def
/npop				% integer npop -
{
	{
	pop
	} repeat
} def
% marking operators
/sw					% ax ay string sw x y 
{
dup length exch stringwidth
exch 5 -1 roll 3 index 1 sub mul add
4 1 roll 3 1 roll 1 sub mul add
} def
/swj				% cx cy fillchar ax ay string swj x y
{
dup 4 1 roll
dup length exch stringwidth 
exch 5 -1 roll 3 index 1 sub mul add
4 1 roll 3 1 roll 1 sub mul add 
6 2 roll /_cnt 0 ddef
{1 index eq {/_cnt _cnt 1 add ddef} if} forall pop
exch _cnt mul exch _cnt mul 2 index add 4 1 roll 2 index add 4 1 roll pop pop
} def
/ss					% ax ay string matrix ss -
{
4 1 roll
	{				% matrix ax ay char 0 0 {proc} -
	2 npop 
	(0) exch 2 copy 0 exch put pop
	gsave
	false charpath currentpoint
	4 index setmatrix
	stroke
	grestore
	moveto
	2 copy rmoveto
	} exch cshow
3 npop
} def
/jss				% cx cy fillchar ax ay string matrix jss -
{
4 1 roll
	{				% cx cy fillchar matrix ax ay char 0 0 {proc} -   
	2 npop 
	(0) exch 2 copy 0 exch put 
	gsave
	_sp eq 
		{
		exch 6 index 6 index 6 index 5 -1 roll widthshow  
		currentpoint
		}
		{
		false charpath currentpoint
		4 index setmatrix stroke
		}ifelse
	grestore
	moveto
	2 copy rmoveto
	} exch cshow
6 npop
} def

% path operators
/sp					% ax ay string sp -
{
	{
	2 npop (0) exch
	2 copy 0 exch put pop
	false charpath
	2 copy rmoveto
	} exch cshow
2 npop
} def
/jsp					% cx cy fillchar ax ay string jsp -
{
	{					% cx cy fillchar ax ay char 0 0 {proc} -
	2 npop 
	(0) exch 2 copy 0 exch put 
	_sp eq 
		{
		exch 5 index 5 index 5 index 5 -1 roll widthshow  
		}
		{
		false charpath
		}ifelse
	2 copy rmoveto
	} exch cshow
5 npop
} def

% path construction operators
/pl				% x y pl x y
{
transform
0.25 sub round 0.25 add exch
0.25 sub round 0.25 add exch
itransform
} def
/setstrokeadjust where
	{
	pop true setstrokeadjust
	/c				% x1 y1 x2 y2 x3 y3 c -
	{
	curveto
	} def
	/C
	/c load def
	/v				% x2 y2 x3 y3 v -
	{
	currentpoint 6 2 roll curveto
	} def
	/V
	/v load def
	/y				% x1 y1 x2 y2 y -
	{
	2 copy curveto
	} def
	/Y
	/y load def
	/l				% x y l -
	{
	lineto
	} def
	/L
	/l load def
	/m				% x y m -
	{
	moveto
	} def
	}
	{%else
	/c
	{
	pl curveto
	} def
	/C
	/c load def
	/v
	{
	currentpoint 6 2 roll pl curveto
	} def
	/V
	/v load def
	/y
	{
	pl 2 copy curveto
	} def
	/Y
	/y load def
	/l
	{
	pl lineto
	} def
	/L
	/l load def
	/m
	{
	pl moveto
	} def
	}ifelse

% graphic state operators
/d					% array phase d -
{
setdash
} def
/cf	{} def			% - cf flatness
/i					% flatness i -
{
dup 0 eq
	{
	pop cf
	} if
setflat
} def
/j					% linejoin j -
{
setlinejoin
} def
/J					% linecap J -
{
setlinecap
} def
/M					% miterlimit M -
{
setmiterlimit
} def
/w					% linewidth w -
{
setlinewidth
} def

% path painting operators
/H					% - H -
{} def
/h					% - h -
{
closepath
} def
/N					% - N -
{
_pola 0 eq 
	{
	_doClip 1 eq {clip /_doClip 0 ddef} if 
	newpath
	} 
	{
	/CRender {N} ddef
	}ifelse
} def
/n					% - n -
{N} def
/F					% - F -
{
_pola 0 eq 
	{
	_doClip 1 eq 
		{
		gsave _pf grestore clip newpath /_lp /none ddef _fc 
		/_doClip 0 ddef
		}
		{
		_pf
		}ifelse
	} 
	{
	/CRender {F} ddef
	}ifelse
} def
/f					% - f -
{
closepath
F
} def
/S					% - S -
{
_pola 0 eq 
	{
	_doClip 1 eq 
		{
		gsave _ps grestore clip newpath /_lp /none ddef _sc 
		/_doClip 0 ddef
		}
		{
		_ps
		}ifelse
	} 
	{
	/CRender {S} ddef
	}ifelse
} def
/s					% - s -
{
closepath
S
} def
/B					% - B -
{
_pola 0 eq 
	{
	_doClip 1 eq 	% F clears _doClip
	gsave F grestore 
		{
		gsave S grestore clip newpath /_lp /none ddef _sc
		/_doClip 0 ddef
		} 
		{
		S
		}ifelse
	}
	{
	/CRender {B} ddef
	}ifelse
} def
/b					% - b -
{
closepath
B
} def
/W					% - W -
{
/_doClip 1 ddef
} def
/*					% - [string] * -
{
count 0 ne 
	{
	dup type (stringtype) eq {pop} if
	} if 
_pola 0 eq {newpath} if
} def

% group operators
/u					% - u -
{} def
/U					% - U -
{} def
/q					% - q -
{
_pola 0 eq {gsave} if
} def
/Q					% - Q -
{
_pola 0 eq {grestore} if
} def
/*u					% - *u -
{
_pola 1 add /_pola exch ddef
} def
/*U					% - *U -
{
_pola 1 sub /_pola exch ddef 
_pola 0 eq {CRender} if
} def
/D					% polarized D -
{pop} def
/*w					% - *w -
{} def
/*W					% - *W -
{} def

% place operators
/`					% matrix llx lly urx ury string ` -
{
/_i save ddef
6 1 roll 4 npop
concat
userdict begin
/showpage {} def
false setoverprint
pop
} def
/~					% - ~ -
{
end
_i restore
} def

% color operators
/O					% flag O -
{
0 ne
/_of exch ddef
/_lp /none ddef
} def
/R					% flag R -
{
0 ne
/_os exch ddef
/_lp /none ddef
} def
/g					% gray g -
{
/_gf exch ddef
/_fc
{ 
_lp /fill ne
	{
	_of setoverprint
	_gf setgray
	/_lp /fill ddef
	} if
} ddef
/_pf
{
_fc
fill
} ddef
/_psf
{
_fc
ashow
} ddef
/_pjsf
{
_fc
awidthshow
} ddef
/_lp /none ddef
} def
/G					% gray G -
{
/_gs exch ddef
/_sc
{
_lp /stroke ne
	{
	_os setoverprint
	_gs setgray
	/_lp /stroke ddef
	} if
} ddef
/_ps
{
_sc
stroke
} ddef
/_pss
{
_sc
ss
} ddef
/_pjss
{
_sc
jss
} ddef
/_lp /none ddef
} def
/k					% cyan magenta yellow black k -
{
_cf astore pop
/_fc
{
_lp /fill ne
	{
	_of setoverprint
	_cf aload pop setcmykcolor
	/_lp /fill ddef
	} if
} ddef
/_pf
{
_fc
fill
} ddef
/_psf
{
_fc
ashow
} ddef
/_pjsf
{
_fc
awidthshow
} ddef
/_lp /none ddef
} def
/K					% cyan magenta yellow black K -
{
_cs astore pop
/_sc
{
_lp /stroke ne
	{
	_os setoverprint
	_cs aload pop setcmykcolor
	/_lp /stroke ddef
	} if
} ddef
/_ps
{
_sc
stroke
} ddef
/_pss
{
_sc
ss
} ddef
/_pjss
{
_sc
jss
} ddef
/_lp /none ddef
} def
/x					% cyan magenta yellow black name gray x -
{
/_gf exch ddef
findcmykcustomcolor
/_if exch ddef
/_fc
{ 
_lp /fill ne
	{
	_of setoverprint
	_if _gf 1 exch sub setcustomcolor
	/_lp /fill ddef
	} if
} ddef
/_pf
{
_fc
fill
} ddef
/_psf
{
_fc
ashow
} ddef
/_pjsf
{
_fc
awidthshow
} ddef
/_lp /none ddef
} def
/X					% cyan magenta yellow black name gray X -
{
/_gs exch ddef
findcmykcustomcolor
/_is exch ddef
/_sc
{
_lp /stroke ne
	{
	_os setoverprint
	_is _gs 1 exch sub setcustomcolor
	/_lp /stroke ddef
	} if
} ddef
/_ps
{
_sc
stroke
} ddef
/_pss
{
_sc
ss
} ddef
/_pjss
{
_sc
jss
} ddef
/_lp /none ddef
} def

% locked object operator
/A					% value A -
{
pop
} def

currentdict readonly pop end
setpacking

% annotate page operator
/annotatepage
{
} def
%%EndResource
%/showpage{}def
/copypage{}def
18 8 translate
[1 0 0 1 0 neg 0 neg] concat
%AI3-Grid.0 18 18 3 0.833333 0.833333 0.833333 3
%%EndProlog
%%BeginSetup
Adobe_cmykcolor /initialize get exec
Adobe_cshow /initialize get exec
Adobe_customcolor /initialize get exec
Adobe_typography_AI3 /initialize get exec
Adobe_IllustratorA_AI3 /initialize get exec
[
39/quotesingle 96/grave 130/quotesinglbase 131/florin 132/quotedblbase
133/ellipsis 134/dagger 135/daggerdbl 136/circumflex 137/perthousand 
138/Scaron 139/guilsinglleft 140/OE 145/quoteleft 146/quoteright 
147/quotedblleft 148/quotedblright 149/bullet 150/endash 151/emdash 
152/tilde 153/trademark 154/scaron 155/guilsinglright 156/oe 157/dotlessi 
159/Ydieresis 164/currency 166/brokenbar 168/dieresis 169/copyright 
170/ordfeminine 172/logicalnot 174/registered 175/macron 176/ring 
177/plusminus 178/twosuperior 179/threesuperior 180/acute 181/mu 
183/periodcentered 184/cedilla 185/onesuperior 186/ordmasculine 
188/onequarter 189/onehalf 190/threequarters 192/Agrave 193/Aacute 
194/Acircumflex 195/Atilde 196/Adieresis 197/Aring 198/AE 199/Ccedilla 
200/Egrave 201/Eacute 202/Ecircumflex 203/Edieresis 204/Igrave 205/Iacute 
206/Icircumflex 207/Idieresis 208/Eth 209/Ntilde 210/Ograve 211/Oacute 
212/Ocircumflex 213/Otilde 214/Odieresis 215/multiply 216/Oslash 
217/Ugrave 218/Uacute 219/Ucircumflex 220/Udieresis 221/Yacute 222/Thorn 
223/germandbls 224/agrave 225/aacute 226/acircumflex 227/atilde 228/adieresis 
229/aring 230/ae 231/ccedilla 232/egrave 233/eacute 234/ecircumflex 
235/edieresis 236/igrave 237/iacute 238/icircumflex 239/idieresis 
240/eth 241/ntilde 242/ograve 243/oacute 244/ocircumflex 245/otilde 
246/odieresis 247/divide 248/oslash 249/ugrave 250/uacute 251/ucircumflex 
252/udieresis 253/yacute 254/thorn 255/ydieresis
TE
%AI3_BeginEncoding: _Times-Roman Times-Roman
[/_Times-Roman/Times-Roman 0 0 1 TZ
%AI3_EndEncoding
%AI3_BeginEncoding: _Times-Italic Times-Italic
[/_Times-Italic/Times-Italic 0 0 1 TZ
%AI3_EndEncoding
%AI3_BeginEncoding: _Times-BoldItalic Times-BoldItalic
[/_Times-BoldItalic/Times-BoldItalic 0 0 1 TZ
%AI3_EndEncoding
/_AI3_savepage save def
%%EndSetup
0 A
0 To
1.4414 0 0 1.3269 323.5681 694.2004 0 Tp
TP
-26.6192 0 Td
0 Tr
0 O
0 g
0 i 0 J 0 j 1 w 4 M []0 d
%AI3_Note:
0 D
/_Times-Italic 14 Tf
0 Ts
100.0008 Tz
0 Tt
0 TA
0 0 5 TC
100 100 200 TW
0 0 0 Ti
1 Ta
0 Tq
0 0 Tl
0 Tc
0 Tw
(H) Tx 
/_Times-Roman 14 Tf
100 Tz
( \(Tesla\)) Tx 
(\r) TX 
TO
0 R
0 G
0.25 w [1 2 ]0 d
111.8294 637.3034 m
535.3101 637.3094 l
S
1 w []0 d
134.1709 637.3038 m
134.171 631.5983 l
S
134.1796 113.3273 m
134.1795 119.0328 l
S
0 To
0 -1.3269 1.4414 0 127.4395 648.4493 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
2 Ta
(0.6) Tx 
(\r) TX 
TO
0 R
0 G
178.7099 637.3044 m
178.71 631.5989 l
S
178.7186 113.3279 m
178.7185 119.0334 l
S
0 To
0 -1.3269 1.4414 0 171.9785 648.4499 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(0.8) Tx 
(\r) TX 
TO
0 R
0 G
223.2489 637.305 m
223.249 631.5995 l
S
223.2576 113.3286 m
223.2575 119.0341 l
S
0 To
0 -1.3269 1.4414 0 216.5174 648.4505 0 Tp
TP
-7 0 Td
0 Tr
0 O
0 g
(1) Tx 
(\r) TX 
TO
0 R
0 G
267.7879 637.3056 m
267.788 631.6001 l
S
267.7966 113.3292 m
267.7965 119.0347 l
S
0 To
0 -1.3269 1.4414 0 261.0564 648.4512 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(1.2) Tx 
(\r) TX 
TO
0 R
0 G
312.471 637.3062 m
312.4711 631.6008 l
S
312.4797 113.3298 m
312.4796 119.0353 l
S
0 To
0 -1.3269 1.4414 0 305.7395 648.4518 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(1.4) Tx 
(\r) TX 
TO
0 R
0 G
357.01 637.3069 m
357.0101 631.6014 l
S
357.0187 113.3305 m
357.0186 119.0359 l
S
0 To
0 -1.3269 1.4414 0 350.2785 648.4524 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(1.6) Tx 
(\r) TX 
TO
0 R
0 G
401.549 637.3075 m
401.5491 631.602 l
S
401.5577 113.3311 m
401.5576 119.0366 l
S
0 To
0 -1.3269 1.4414 0 394.8175 648.453 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(1.8) Tx 
(\r) TX 
TO
0 R
0 G
446.088 637.3081 m
446.0881 631.6027 l
S
446.0967 113.3317 m
446.0966 119.0372 l
S
0 To
0 -1.3269 1.4414 0 439.3565 648.4537 0 Tp
TP
-7 0 Td
0 Tr
0 O
0 g
(2) Tx 
(\r) TX 
TO
0 R
0 G
490.7711 637.3088 m
490.7712 631.6033 l
S
490.7798 113.3323 m
490.7797 119.0378 l
S
0 To
0 -1.3269 1.4414 0 484.0396 648.4543 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(2.2) Tx 
(\r) TX 
TO
0 R
0 G
535.3101 637.3094 m
535.3101 631.6039 l
S
535.3188 113.333 m
535.3187 119.0385 l
S
0 To
0 -1.3269 1.4414 0 528.5786 648.4549 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(2.4) Tx 
(\r) TX 
TO
0 R
0 G
111.8294 637.3034 m
118.0274 637.3035 l
S
535.3101 637.3094 m
529.1121 637.3093 l
S
0 To
0 -1.3269 1.4414 0 84.9186 637.3031 0 Tp
TP
-3.5 0 Td
0 Tr
0 O
0 g
1 Ta
(0) Tx 
(\r) TX 
TO
0 R
0 G
111.8305 571.7566 m
118.0285 571.7567 l
S
535.3111 571.7626 m
529.1132 571.7625 l
S
0 To
0 -1.3269 1.4414 0 84.9197 571.7562 0 Tp
TP
-12.25 0 Td
0 Tr
0 O
0 g
(0.05) Tx 
(\r) TX 
TO
0 R
0 G
111.8316 506.3425 m
118.0296 506.3426 l
S
535.3122 506.3484 m
529.1143 506.3484 l
S
0 To
0 -1.3269 1.4414 0 84.9208 506.3421 0 Tp
TP
-8.75 0 Td
0 Tr
0 O
0 g
(0.1) Tx 
(\r) TX 
TO
0 R
0 G
111.8326 440.7957 m
118.0306 440.7958 l
S
535.3133 440.8016 m
529.1153 440.8016 l
S
0 To
0 -1.3269 1.4414 0 84.9219 440.7953 0 Tp
TP
-12.25 0 Td
0 Tr
0 O
0 g
(0.15) Tx 
(\r) TX 
TO
0 R
0 G
111.8337 375.2489 m
118.0317 375.249 l
S
535.3144 375.2548 m
529.1164 375.2547 l
S
0 To
0 -1.3269 1.4414 0 84.923 375.2485 0 Tp
TP
-8.75 0 Td
0 Tr
0 O
0 g
(0.2) Tx 
(\r) TX 
TO
0 R
0 G
111.8348 309.8348 m
118.0328 309.8348 l
S
535.3155 309.8407 m
529.1175 309.8406 l
S
0 To
0 -1.3269 1.4414 0 84.9241 309.8344 0 Tp
TP
-12.25 0 Td
0 Tr
0 O
0 g
(0.25) Tx 
(\r) TX 
TO
0 R
0 G
111.8359 244.2879 m
118.0339 244.288 l
S
535.3166 244.2939 m
529.1186 244.2938 l
S
0 To
0 -1.3269 1.4414 0 84.9251 244.2876 0 Tp
TP
-8.75 0 Td
0 Tr
0 O
0 g
(0.3) Tx 
(\r) TX 
TO
0 R
0 G
111.837 178.8738 m
118.035 178.8739 l
S
535.3177 178.8798 m
529.1197 178.8797 l
S
0 To
0 -1.3269 1.4414 0 84.9262 178.8734 0 Tp
TP
-12.25 0 Td
0 Tr
0 O
0 g
(0.35) Tx 
(\r) TX 
TO
0 R
0 G
111.8381 113.327 m
118.0361 113.3271 l
S
535.3188 113.333 m
529.1208 113.3329 l
S
0 To
0 -1.3269 1.4414 0 84.9273 113.3266 0 Tp
TP
-8.75 0 Td
0 Tr
0 O
0 g
(0.4) Tx 
(\r) TX 
TO
0 R
0 G
111.8294 637.3034 m
111.8381 113.327 l
535.3188 113.333 l
535.3101 637.3094 l
111.8294 637.3034 l
S
0 To
0 -1.3269 1.4414 0 50.6826 375.3809 0 Tp
TP
-15.3536 0 Td
0 Tr
0 O
0 g
/_Times-Italic 14 Tf
100.0008 Tz
(T) Tx 
/_Times-Roman 14 Tf
100 Tz
( \(K\)) Tx 
(\r) TX 
TO
0 To
1.3269 0 0 1.4414 347.2239 42.6145 0 Tp
TP
-99.345 0 Td
0 Tr
(K. A. Park and Robert Joynt, Fig. 2) Tx 
(\r) TX 
TO
0 To
0 -1.3269 1.4414 0 502.209 174.766 0 Tp
TP
-72.8371 0 Td
0 Tr
/_Times-BoldItalic 14 Tf
100.0008 Tz
2 Ta
(H) Tx 
/_Times-Roman 14 Tf
100 Tz
( || ab \(data\)) Tx 
(\r) TX 
TO
0 R
0 G
508.9406 155.2613 m
505.9137 152.4749 l
508.9407 149.6885 l
511.9676 152.475 l
508.9406 155.2613 l
S
508.9406 152.4749 m
508.9406 152.4749 l
S
503.4568 550.1343 m
500.4299 547.3479 l
503.4569 544.5615 l
506.4837 547.348 l
503.4568 550.1343 l
S
503.4568 547.3479 m
503.4568 547.3479 l
S
447.5318 488.5673 m
444.5049 485.7809 l
447.5319 482.9945 l
450.5588 485.781 l
447.5318 488.5673 l
S
447.5319 485.7809 m
447.5319 485.7809 l
S
370.5634 378.0389 m
367.5365 375.2525 l
370.5635 372.4661 l
373.5904 375.2526 l
370.5634 378.0389 l
S
370.5634 375.2525 m
370.5634 375.2525 l
S
333.6643 346.0611 m
330.6374 343.2747 l
333.6644 340.4883 l
336.6913 343.2747 l
333.6643 346.0611 l
S
333.6643 343.2747 m
333.6643 343.2747 l
S
266.7847 288.2091 m
263.7578 285.4227 l
266.7848 282.6363 l
269.8117 285.4228 l
266.7847 288.2091 l
S
266.7847 285.4227 m
266.7847 285.4227 l
S
229.7417 243.3608 m
226.7148 240.5744 l
229.7418 237.788 l
232.7687 240.5744 l
229.7417 243.3608 l
S
229.7417 240.5744 m
229.7417 240.5744 l
S
228.0122 231.6844 m
224.9853 228.898 l
228.0123 226.1116 l
231.0392 228.8981 l
228.0122 231.6844 l
S
228.0123 228.898 m
228.0123 228.898 l
S
188.2304 199.5739 m
185.2035 196.7874 l
188.2304 194.0011 l
191.2573 196.7875 l
188.2304 199.5739 l
S
188.2304 196.7875 m
188.2304 196.7875 l
S
154.7906 170.1172 m
151.7637 167.3307 l
154.7907 164.5444 l
157.8176 167.3308 l
154.7906 170.1172 l
S
154.7906 167.3308 m
154.7906 167.3308 l
S
143.9804 155.9196 m
140.9535 153.1332 l
143.9805 150.3468 l
147.0074 153.1333 l
143.9804 155.9196 l
S
143.9804 153.1332 m
143.9804 153.1332 l
S
141.2419 148.2238 m
138.215 145.4373 l
141.242 142.651 l
144.2688 145.4375 l
141.2419 148.2238 l
S
141.2419 145.4374 m
141.2419 145.4374 l
S
131.2964 144.3758 m
128.2695 141.5893 l
131.2964 138.803 l
134.3233 141.5894 l
131.2964 144.3758 l
S
131.2964 141.5894 m
131.2964 141.5894 l
S
121.351 130.3109 m
118.3241 127.5245 l
121.3511 124.7381 l
124.3779 127.5246 l
121.351 130.3109 l
S
121.351 127.5245 m
121.351 127.5245 l
S
0 To
0 -1.3269 1.4414 0 482.0295 174.7658 0 Tp
TP
-65.8371 0 Td
0 Tr
0 O
0 g
/_Times-BoldItalic 14 Tf
100.0008 Tz
(H) Tx 
/_Times-Roman 14 Tf
100 Tz
( || c \(data\)) Tx 
(\r) TX 
TO
0 R
0 G
488.7611 155.2611 m
488.7611 155.2611 l
488.7612 149.6882 l
S
485.7342 152.4746 m
485.7342 152.4746 l
491.7881 152.4747 l
S
421.8744 529.0361 m
421.8744 529.0361 l
421.8745 523.4633 l
S
418.8475 526.2497 m
418.8475 526.2497 l
424.9013 526.2498 l
S
393.192 448.7608 m
393.192 448.7608 l
393.1921 443.188 l
S
390.1652 445.9743 m
390.1652 445.9743 l
396.219 445.9744 l
S
338.2771 326.1583 m
338.2771 326.1583 l
338.2772 320.5855 l
S
335.2502 323.3719 m
335.2502 323.3719 l
341.304 323.3719 l
S
298.7839 268.8375 m
298.7839 268.8375 l
298.784 263.2647 l
S
295.757 266.051 m
295.757 266.051 l
301.8109 266.0511 l
S
301.5226 266.1838 m
301.5226 266.1838 l
301.5227 260.611 l
S
298.4957 263.3973 m
298.4957 263.3973 l
304.5496 263.3974 l
S
279.0372 244.5557 m
279.0372 244.5557 l
279.0373 238.9829 l
S
276.0104 241.7692 m
276.0104 241.7692 l
282.0642 241.7693 l
S
267.3621 238.1866 m
267.3621 238.1866 l
267.3622 232.6138 l
S
264.3352 235.4001 m
264.3352 235.4001 l
270.3891 235.4002 l
S
232.337 197.3189 m
232.337 197.3189 l
232.3371 191.7461 l
S
229.3101 194.5324 m
229.3101 194.5324 l
235.3639 194.5325 l
S
237.6701 196.1247 m
237.6701 196.1247 l
237.6702 190.5519 l
S
234.6433 193.3383 m
234.6433 193.3383 l
240.6971 193.3384 l
S
229.5984 189.7557 m
229.5984 189.7557 l
229.5986 184.1829 l
S
226.5716 186.9693 m
226.5716 186.9693 l
232.6254 186.9694 l
S
222.3916 183.254 m
222.3916 183.254 l
222.3917 177.6812 l
S
219.3647 180.4676 m
219.3647 180.4676 l
225.4186 180.4677 l
S
215.1848 175.6908 m
215.1848 175.6908 l
215.1849 170.118 l
S
212.1579 172.9044 m
212.1579 172.9044 l
218.2117 172.9044 l
S
209.8517 171.8429 m
209.8517 171.8429 l
209.8518 166.27 l
S
206.8248 169.0564 m
206.8248 169.0564 l
212.8787 169.0565 l
S
201.78 164.147 m
201.78 164.147 l
201.7801 158.5742 l
S
198.7532 161.3605 m
198.7532 161.3605 l
204.807 161.3606 l
S
195.438 159.1048 m
195.438 159.1048 l
195.4381 153.532 l
S
192.4111 156.3184 m
192.4111 156.3184 l
198.465 156.3184 l
S
191.8346 151.409 m
191.8346 151.409 l
191.8347 145.8362 l
S
188.8078 148.6225 m
188.8078 148.6225 l
194.8616 148.6226 l
S
180.1596 137.3441 m
180.1596 137.3441 l
180.1597 131.7713 l
S
177.1327 134.5577 m
177.1327 134.5577 l
183.1866 134.5578 l
S
174.6824 130.9751 m
174.6824 130.9751 l
174.6825 125.4023 l
S
171.6556 128.1887 m
171.6556 128.1887 l
177.7094 128.1887 l
S
0 To
0 -1.3269 1.4414 0 461.85 174.7655 0 Tp
TP
-85.2819 0 Td
0 Tr
0 O
0 g
/_Times-BoldItalic 14 Tf
100.0008 Tz
(H) Tx 
/_Times-Roman 14 Tf
100 Tz
( || ab \(theory\)) Tx 
(\r) TX 
TO
0 R
0 G
468.5815 163.62 m
468.5821 130.1831 l
S
535.3109 587.8176 m
532.7164 584.3677 l
528.8248 579.0602 l
524.9331 573.7527 l
521.0414 568.4452 l
517.0056 563.2704 l
513.114 557.9629 l
509.0782 552.6555 l
505.1865 547.348 l
501.1507 542.0405 l
497.1149 536.733 l
493.0791 531.4255 l
489.0433 526.118 l
485.0075 520.8105 l
480.9716 515.6357 l
476.7917 510.3282 l
472.7559 505.0207 l
468.5759 499.7132 l
464.396 494.4057 l
460.216 489.0982 l
456.1803 483.7907 l
451.8562 478.4832 l
447.6762 473.1757 l
443.4963 468.001 l
439.3163 462.6935 l
434.9922 457.386 l
430.6681 452.0785 l
426.4882 446.771 l
422.1641 441.4635 l
417.84 436.156 l
413.516 430.8485 l
409.0477 425.541 l
404.7236 420.3662 l
400.2554 415.0587 l
395.9313 409.7512 l
391.4631 404.4437 l
386.9949 399.1362 l
382.5267 393.8287 l
378.0584 388.5212 l
373.4461 383.2137 l
368.9779 377.9062 l
364.3655 372.7314 l
359.7531 367.4239 l
355.1407 362.1164 l
350.5284 356.8089 l
345.916 351.5014 l
341.1595 346.1939 l
336.5472 340.8864 l
331.7906 335.5789 l
327.0341 330.2714 l
322.2776 325.0966 l
317.5211 319.7891 l
312.6205 314.4816 l
307.7199 309.1741 l
302.9634 303.8666 l
298.0627 298.5591 l
293.0179 293.2516 l
288.1173 287.9441 l
283.2167 282.6366 l
278.1719 277.4617 l
273.1271 272.1542 l
268.0823 266.8467 l
262.8934 261.5392 l
257.8486 256.2317 l
252.6597 250.9242 l
247.4708 245.6167 l
242.2818 240.3092 l
236.9488 235.0017 l
231.7599 229.8269 l
226.4268 224.5194 l
221.0938 219.2119 l
215.6166 213.9044 l
210.2835 208.5968 l
204.8063 203.2893 l
199.185 197.9818 l
193.7078 192.6743 l
188.0864 187.3668 l
182.4651 182.192 l
176.8438 176.8844 l
171.2224 171.5769 l
165.4569 166.2694 l
159.6915 160.9619 l
153.7819 155.6544 l
148.0164 150.3469 l
142.1068 145.0393 l
136.053 139.7318 l
129.9992 134.557 l
123.9455 129.2495 l
117.8917 123.942 l
111.838 118.7671 l
S
0 To
0 -1.3269 1.4414 0 441.6706 174.7652 0 Tp
TP
-78.2819 0 Td
0 Tr
0 O
0 g
/_Times-BoldItalic 14 Tf
100.0008 Tz
(H) Tx 
/_Times-Roman 14 Tf
100 Tz
( || c \(theory\)) Tx 
(\r) TX 
TO
0 R
0 G
[6 3 ]0 d
448.402 163.6197 m
448.4026 130.1828 l
S
167.6199 113.3278 m
170.6468 116.7777 l
175.2591 122.3505 l
180.0156 127.9234 l
184.7721 133.629 l
189.5286 139.3345 l
194.2851 145.1728 l
198.8975 151.011 l
203.6539 156.9819 l
208.4105 162.9529 l
213.1669 168.9238 l
217.9234 175.0274 l
222.5358 181.2637 l
227.2923 187.5 l
232.0487 193.7363 l
236.8052 200.238 l
241.5617 206.607 l
246.1741 213.2413 l
250.9305 219.8757 l
255.687 226.6427 l
260.4435 233.4098 l
265.2 240.3095 l
269.8123 247.3419 l
274.5688 254.507 l
279.3252 261.8048 l
284.0817 269.1026 l
288.8382 276.5331 l
293.4505 284.0962 l
298.207 291.7921 l
302.9635 299.488 l
307.7199 307.3165 l
312.4763 315.4104 l
317.0887 323.3716 l
321.8451 331.5982 l
326.6016 339.9575 l
331.358 348.3167 l
336.1145 356.8087 l
340.7268 365.4333 l
345.4832 374.1907 l
350.2397 383.0807 l
354.9961 391.9707 l
359.7525 400.9934 l
364.3648 410.2815 l
369.1213 419.5696 l
373.8777 428.8576 l
378.6342 438.4111 l
383.3906 447.9645 l
388.0029 457.7834 l
392.7593 467.6022 l
397.5157 477.5537 l
402.2722 487.6379 l
407.0286 497.7221 l
411.6408 508.0716 l
416.3973 518.4212 l
421.1537 528.9035 l
425.9101 539.5184 l
430.6665 550.266 l
435.4229 561.1463 l
440.0352 572.0266 l
444.7916 583.1723 l
449.548 594.318 l
454.3044 605.5963 l
459.0608 617.0074 l
463.6731 628.4184 l
467.2764 637.3084 l
S
%%PageTrailer
_AI3_savepage restore
gsave annotatepage grestore
%%Trailer
Adobe_IllustratorA_AI3 /terminate get exec
Adobe_typography_AI3 /terminate get exec
Adobe_customcolor /terminate get exec
Adobe_cshow /terminate get exec
Adobe_cmykcolor /terminate get exec
Adobe_packedarray /terminate get exec
%%EndDocument
1 #C
statusdict begin /manualfeed false store end
EJ RS
%%PageTrailer
%%PageResources: 
2394 3231 0 0 CB
%%Trailer
SVDoc restore
end
%%Pages: 1
%%DocumentSuppliedResources: procset Win35Dict 3 1

%%DocumentNeededResources: 
%%EOF


==> hzplot <==
%!PS-Adobe-3.0
%%Creator: Windows PSCRIPT
%%Title: HZPLOT.AI
%%BoundingBox: 18 9 593 784
%%DocumentNeededResources: (atend)
%%DocumentSuppliedResources: (atend)
%%Pages: (atend)
%%BeginResource: procset Win35Dict 3 1
/Win35Dict 60 dict def Win35Dict begin/bd{bind def}bind def/in{72
mul}bd/ed{exch def}bd/ld{load def}bd/tr/translate ld/gs/gsave ld/gr
/grestore ld/fPP false def/SS{fPP{/SV save def}{gs}ifelse}bd/RS{fPP{SV
restore}{gr}ifelse}bd/EJ{gsave showpage grestore}bd/#C{userdict begin
/#copies ed end}bd/FEbuf 2 string def/FEglyph(G  )def/FE{1 exch{dup
16 FEbuf cvrs FEglyph exch 1 exch putinterval 1 index exch FEglyph
cvn put}for}bd/SM{/iRes ed/cyP ed/cxPg ed/cyM ed/cxM ed 0 ne{0 cyP
72 mul 100 div tr -90 rotate}if pop}bd/CB{moveto/dy ed/dx ed dx 0 rlineto
0 dy rlineto dx neg 0 rlineto closepath clip newpath}bd/ErrHandler{errordict
dup maxlength exch length gt dup{errordict begin}if/errhelpdict 12
dict def errhelpdict begin/stackunderflow(operand stack underflow)def
/undefined(this name is not defined in a dictionary)def/VMerror(you have used up all the printer's memory)def
/typecheck(operator was expecting a different type of operand)def
/ioerror(input/output error occured)def end{end}if errordict begin
/handleerror{$error begin newerror{/newerror false def showpage 72
72 scale/x .25 def/y 9.6 def/Helvetica findfont .2 scalefont setfont
x y moveto(Offending Command = )show/command load{dup type/stringtype
ne{(max err string)cvs}if show}exec/y y .2 sub def x y moveto(Error = )show
errorname{dup type dup( max err string )cvs show( : )show/stringtype
ne{( max err string )cvs}if show}exec errordict begin errhelpdict errorname
known{x 1 add y .2 sub moveto errhelpdict errorname get show}if end
/y y .4 sub def x y moveto(Stack =)show ostack{/y y .2 sub def x 1
add y moveto dup type/stringtype ne{( max err string )cvs}if show}forall
showpage}if end}def end}bd end
%%EndResource
/SVDoc save def
%%EndProlog
%%BeginSetup
Win35Dict begin
ErrHandler
statusdict begin 0 setjobtimeout end
statusdict begin statusdict /jobname (HZPLOT.AI) put end
/oldDictCnt countdictstack def {}stopped 
{ countdictstack oldDictCnt lt { Win35Dict begin } 
{1 1 countdictstack oldDictCnt sub {pop end } for } ifelse } if 
/oldDictCnt countdictstack def {letter
}stopped 
{ countdictstack oldDictCnt lt { Win35Dict begin } 
{1 1 countdictstack oldDictCnt sub {pop end } for } ifelse } if 
[
{mark 1.0 1.0 .98 .9 .82 .68 .56 .48 .28 .1 .06 .0 counttomark dup 3 add -1 roll exch 2 sub mul dup floor cvi dup 3 1 roll sub exch dup  3 add index exch 2 add index dup 4 1 roll sub mul add counttomark 1 add 1 roll  cleartomark } bind
/exec load currenttransfer /exec load] cvx settransfer
%%EndSetup
%%Page: 1 1
%%PageResources: (atend)
SS
0 0 25 11 798 1100 300 SM
2394 3231 0 0 CB
%%BeginDocument: Adobe Illustrator(TM) for Windows, version
%!PS-Adobe-3.0 EPSF-3.0
%%Creator: Adobe Illustrator(TM) for Windows, version 4.0
%%For: (Robert J. Joynt                         ) (Physics Dept.  UW - Madison             )
%%CreationDate: (12/7/94) (4:54 PM)
%%BoundingBox: 41 39 546 711
%%DocumentProcessColors: Black
%%DocumentFonts: Times-Roman
%%+ Times-Italic
%%DocumentSuppliedResources: procset Adobe_packedarray 2.0 0
%%+ procset Adobe_cmykcolor 1.1 0
%%+ procset Adobe_cshow 1.1 0
%%+ procset Adobe_customcolor 1.0 0
%%+ procset Adobe_typography_AI3 1.0 0
%%+ procset Adobe_IllustratorA_AI3 1.0 0
%AI3_ColorUsage: Black&White
%AI3_TemplateBox: 300 225 300 225
%AI3_TileBox: 0 0 575 775
%AI3_DocumentPreview: Header
%%Template:
%%PageOrigin:0 0
%%AI3_PaperRect:-18 784 594 -8
%%AI3_Margin:18 -9 -19 8
%%EndComments
%%BeginProlog
%%BeginResource: procset Adobe_packedarray 2.0 0
%%Title: (Packed Array Operators)
%%Version: 2.0 
%%CreationDate: (8/2/90) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

userdict /Adobe_packedarray 5 dict dup begin put
/initialize			% - initialize -
{
/packedarray where
	{
	pop
	}
	{
	Adobe_packedarray begin
	Adobe_packedarray
		{
		dup xcheck
			{
			bind
			} if
		userdict 3 1 roll put
		} forall
	end
	} ifelse
} def
/terminate			% - terminate -
{
} def
/packedarray		% arguments count packedarray array
{
array astore readonly
} def
/setpacking			% boolean setpacking -
{
pop
} def
/currentpacking		% - setpacking boolean
{
false
} def
currentdict readonly pop end
%%EndResource
Adobe_packedarray /initialize get exec
%%BeginResource: procset Adobe_cmykcolor 1.1 0
%%Title: (CMYK Color Operators)
%%Version: 1.1 
%%CreationDate: (1/23/89) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

currentpacking true setpacking
userdict /Adobe_cmykcolor 4 dict dup begin put
/initialize			% - initialize -
{
/setcmykcolor where
	{
	pop
	}
	{
	userdict /Adobe_cmykcolor_vars 2 dict dup begin put
	/_setrgbcolor
		/setrgbcolor load def
	/_currentrgbcolor
		/currentrgbcolor load def
	Adobe_cmykcolor begin
	Adobe_cmykcolor
		{
		dup xcheck
			{
			bind
			} if
		pop pop
		} forall
	end
	end
	Adobe_cmykcolor begin
	} ifelse
} def
/terminate			% - terminate -
{
currentdict Adobe_cmykcolor eq
	{
	end
	} if
} def
/setcmykcolor		% cyan magenta yellow black setcmykcolor -
{
1 sub 4 1 roll
3
	{
	3 index add neg dup 0 lt
		{
		pop 0
		} if
	3 1 roll
	} repeat
Adobe_cmykcolor_vars /_setrgbcolor get exec
pop
} def 
/currentcmykcolor	% - currentcmykcolor cyan magenta yellow black
{
Adobe_cmykcolor_vars /_currentrgbcolor get exec
3
	{
	1 sub neg 3 1 roll
	} repeat
0
} def
currentdict readonly pop end
setpacking

%%EndResource
%%BeginResource: procset Adobe_cshow 1.1 0
%%Title: (cshow Operator)
%%Version: 1.1 
%%CreationDate: (1/23/89) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

currentpacking true setpacking
userdict /Adobe_cshow 3 dict dup begin put
/initialize			% - initialize -
{
/cshow where
	{
	pop
	}
	{
	userdict /Adobe_cshow_vars 1 dict dup begin put
	/_cshow		% - _cshow proc
		{} def
	Adobe_cshow begin
	Adobe_cshow
		{
		dup xcheck
			{
			bind
			} if
		userdict 3 1 roll put
		} forall
	end
	end
	} ifelse
} def
/terminate			% - terminate -
{
} def
/cshow				% proc string cshow -
{
exch
Adobe_cshow_vars
	exch /_cshow
	exch put
	{
	0 0 Adobe_cshow_vars /_cshow get exec
	} forall
} def
currentdict readonly pop end
setpacking

%%EndResource
%%BeginResource: procset Adobe_customcolor 1.0 0
%%Title: (Custom Color Operators)
%%Version: 1.0 
%%CreationDate: (5/9/88) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

currentpacking true setpacking
userdict /Adobe_customcolor 5 dict dup begin put
/initialize			% - initialize -
{
/setcustomcolor where
	{
	pop
	}
	{
	Adobe_customcolor begin
	Adobe_customcolor
		{
		dup xcheck
			{
			bind
			} if
		pop pop
		} forall
	end
	Adobe_customcolor begin
	} ifelse
} def
/terminate			% - terminate -
{
currentdict Adobe_customcolor eq
	{
	end
	} if
} def
/findcmykcustomcolor	% cyan magenta yellow black name findcmykcustomcolor object
{
5 packedarray
}  def
/setcustomcolor		% object tint setcustomcolor -
{
exch
aload pop pop
4
	{
	4 index mul 4 1 roll
	} repeat
5 -1 roll pop
setcmykcolor
} def
/setoverprint		% boolean setoverprint -
{
pop
} def
currentdict readonly pop end
setpacking

%%EndResource
%%BeginResource: procset Adobe_typography_AI3 1.0 0
%%Title: (Typography Operators)
%%Version: 1.0 
%%CreationDate:(5/31/90) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

currentpacking true setpacking
userdict /Adobe_typography_AI3 46 dict dup begin put
/initialize			% - initialize -
{
/TZ
 where
	{
	pop
	}
	{
	Adobe_typography_AI3 begin
	Adobe_typography_AI3
		{
		dup xcheck
			{
			bind
			} if
		pop pop
		} forall
	end
	Adobe_typography_AI3 begin
	} ifelse
} def
/terminate			% - terminate -
{
currentdict Adobe_typography_AI3 eq
	{
	end
	} if
} def

% [ number value stream [ array for encoding modification ] modifyEncoding ==> [ modified array ]
/modifyEncoding
{
	/_tempEncode exch ddef
	
	% pointer for sequential encodings
	/_pntr 0 ddef
	
	{
		% get bottom object
		counttomark -1 roll

		% is it a mark ?
		dup type dup /marktype eq 		
		{
			% exit
			pop pop exit
		}
		{
			% ... object ... type ....

			% insert if a nametype
			/nametype eq
			{
				% insert the name at _pntr and increment pointer
				_tempEncode /_pntr dup load dup 3 1 roll 1 add ddef 3 -1 roll
				put
			}
			{
				% reset _pntr if it's a number
				/_pntr exch ddef					
			}
			ifelse
		}
		ifelse
	}
	loop	
	
	% return the modified encoding
	_tempEncode
}
def

/TE	% Set std platform encoding 	% (encoding pairs) TE -
{
	StandardEncoding 256 array copy modifyEncoding 
	/_nativeEncoding exch def
} def

% re-define font
% expected arguments
% for 'normal fonts : 
%	[ /_Helvetica-Bold/Helvetica-Bold direction fontScript defaultEncoding TZ
%
% for cartographic, pictographic, and expert fonts :
% 	[ ... number value stream ... /_Helvetica-Bold/Helvetica-Bold 
%	direction fontScript defaultEncoding TZ
/TZ		
{
	% platform dependent coding flag
	/_useNativeEncoding exch def

	% pop fontScript & direction
	pop pop
	
	% create a new dictionary with length
	% equal to original dictionary length + 2
	% copy all the key/value pairs except FID
	findfont dup length 2 add dict
	
	begin
	
		% copy all the values but the FID
		% into the new dictionary
		mark exch
		{
			1 index /FID ne { def } if cleartomark mark
		}
		forall
		% discard last mark
		pop
		
		% define FontName
		/FontName exch def
		
		% if no re-encoding stream is present
		% then if the base encoding vector of the font
		% is the same as StandardEncoding
		% and the use platform encoding flag is true
		% then install AI platform encoding
		% else leave the base encoding in effect

		counttomark 0 eq
		{
			Encoding StandardEncoding eq 1 _useNativeEncoding eq and
			{
				/Encoding _nativeEncoding def
			}
			if
			% clean up
			cleartomark
		}
		{	
			% custom encoding to be done
			% start off with a copy of the font's standard encoding
			/Encoding load 256 array copy 
			modifyEncoding /Encoding exch def
		}
		ifelse		
		FontName currentdict
	end
	
	% register the new font
	definefont pop
}
def

% text painting operators
/tr					% string tr ax ay string 
{
_ax _ay 3 2 roll
} def
/trj				% string trj cx cy fillchar ax ay string 
{
_cx _cy _sp _ax _ay 6 5 roll
} def

/a0
{
/Tx	% text							% textString Tx -
	{
	dup 
	currentpoint 3 2 roll
	tr _psf
	newpath moveto
	tr _ctm _pss
	} ddef
/Tj	% justified text				% textString Tj -
	{
	dup
	currentpoint 3 2 roll
	trj _pjsf
	newpath moveto
	trj _ctm _pjss
	} ddef
	
} def
/a1
{
W B
} def

/e0
{
/Tx	% text							% textString Tx -
	{
	tr _psf
	} ddef
/Tj	% justified text				% textString Tj -
	{
	trj _pjsf
	} ddef
} def

/e1
{
W F 
} def


/i0
{
/Tx	% text							% textString Tx -
	{
	tr sp
	} ddef
/Tj	% justified text				% textString Tj -
	{
	trj jsp
	} ddef
} def

/o0
{
/Tx	% text							% textString Tx -
	{
	tr sw rmoveto
	} ddef
/Tj	% justified text				% textString Tj -
	{
	trj swj rmoveto
	} ddef
} def

/r0
{
/Tx	% text							% textString Tx -
	{
	tr _ctm _pss
	} ddef
/Tj	% justified text				% textString Tj -
	{
	trj _ctm _pjss
	} ddef
} def
/r1
{
W S
} def

% font operators

% Binding
/To	% begin text 					% bindType To -
{
	pop _ctm currentmatrix pop
} def

/TO	% end text					% TO -
{
	Te _ctm setmatrix newpath
} def

% Text paths
/Tp	% begin text path				% a b c d tx ty startPt Tp -
{
	pop _tm astore pop _ctm setmatrix 
	2 dict begin /W {} def /h {} def
} def

/TP	% end text path					% TP -
{
	end
	iTm 0 0 moveto
} def

% Render mode & matrix operators
/Tr	% begin render					% render Tr - 
{
	Te currentpoint newpath moveto
	dup 8 eq {pop 0} {dup 9 eq {pop 1} if} ifelse
	dup /_render exch ddef
	_renderStart exch get load exec
} def

/iTm % internal set text matrix		% - iTm -	(uses _tm as implicit argument)
{
_ctm setmatrix _tm concat 0 _rise translate _hs 1 scale
} def

/Tm % set text matrix				% a b c d tx ty Tm -
{
_tm astore pop iTm 0 0 moveto
} def

/Td % translate text matrix 		% tx ty Td -
{
_mtx translate _tm _tm concatmatrix pop iTm 0 0 moveto
} def

/Te	% end render					% - Te -
{
	_render -1 eq {} {_renderEnd _render get dup null ne {load exec} {pop} ifelse} ifelse
	/_render -1 ddef
} def


% Attributes
/Ta	% set alignment					% alignment Ta -
{
pop
} def

/Tf	% set font name and size		% fontname size Tf -
{
dup 1000 div /_fScl exch ddef
exch findfont exch scalefont setfont
} def

/Tl	% set leading					% leading paragraphLeading Tl -
{
pop
0 exch _leading astore pop
} def

/Tt	% set user tracking				% userTracking Tt -
{
pop
} def

/TW % set word spacing				% minSpace optSpace maxSpace TW -
{
3 npop
} def

/Tw	% set computed word spacing		% wordSpace Tw
{
/_cx exch ddef
} def

/TC % set character spacing			% minSpace optSpace maxSpace TC -
{
3 npop
} def

/Tc	% set computed char spacing 	% charSpace Tc -
{
/_ax exch ddef
} def

/Ts % set super/subscripting (rise)	% rise Ts -
{
/_rise exch ddef
currentpoint
iTm
moveto
} def

/Ti	% set indentation				% firstStartIndent otherStartIndent stopIndent Ti -
{
3 npop
} def

/Tz % set horizontal scaling		% scalePercent Tz -
{
100 div /_hs exch ddef
iTm
} def

/TA % set pairwise kerning			% autoKern TA -
									%	autoKern = 0 -> no pair kerning
									%			 = 1 -> automatic pair kerning
{
pop
} def

/Tq % set hanging quotes			% hangingQuotes Tq -
									%	hangingQuotes 	= 0 -> no hanging quotes
									%			 		= 1 -> hanging quotes
{
pop
} def


% Text Bodies
/TX {pop} def

%/Tx	% non-justified text			% textString Tx -
%/Tj	% justified text				% textString Tj -

/Tk	% kern							% autoKern kernValue Tk -
									%  	autoKern = 0 -> manual kern, = 1 -> auto kern
									%	kernValue = kern value in em/1000 space
{
exch pop _fScl mul neg 0 rmoveto
} def
/TK	% non-printing kern				% autoKern kernValue TK -
{
2 npop
} def

/T* % carriage return & line feed	% - T* -
{
_leading aload pop neg Td
} def

/T*- % carriage return & negative line feed	% - T*- -
{
_leading aload pop Td
} def

/T-	% print a discretionary hyphen	% - T- -
{
_hyphen Tx
} def

/T+	% discretionary hyphen hyphen	% - T+ -
{} def

/TR	% reset pattern matrix 			% a b c d tx ty TR -
{
_ctm currentmatrix pop 	
_tm astore pop 
iTm 0 0 moveto 
} def

/TS	% special chars					% textString justified TS -
{
0 eq {Tx} {Tj} ifelse
} def

currentdict readonly pop end
setpacking

%%EndResource
%%BeginResource: procset Adobe_IllustratorA_AI3 1.0 0
%%Title: (Adobe Illustrator (R) Version 3.0 Abbreviated Prolog)
%%Version: 1.0 
%%CreationDate: (7/22/89) ()
%%Copyright: ((C) 1987-1990 Adobe Systems Incorporated All Rights Reserved)

currentpacking true setpacking
userdict /Adobe_IllustratorA_AI3 61 dict dup begin put
% initialization
/initialize				% - initialize -
{
userdict /Adobe_IllustratorA_AI3_vars 46 dict dup begin put

% paint operands
/_lp /none def
/_pf {} def
/_ps {} def
/_psf {} def
/_pss {} def
/_pjsf {} def
/_pjss {} def
/_pola 0 def
/_doClip 0 def

% paint operators
/cf	currentflat def	% - cf flatness

% typography operands
/_tm matrix def
/_renderStart [/e0 /r0 /a0 /o0 /i0 /i0 /i0 /i0] def 
/_renderEnd [null null null null /e1 /r1 /a1 /clip] def
/_render -1 def
/_rise 0 def
/_ax 0 def			% x character spacing	(_ax, _ay, _cx, _cy follows awidthshow naming convention)
/_ay 0 def			% y character spacing
/_cx 0 def			% x word spacing
/_cy 0 def			% y word spacing
/_leading [0 0] def
/_ctm matrix def
/_mtx matrix def
/_sp 16#020 def
/_hyphen (-) def
/_fScl 0 def
/_cnt 0 def
/_hs 1 def
/_nativeEncoding 0 def
/_useNativeEncoding 0 def
/_tempEncode 0 def
/_pntr 0 def

% typography operators
/Tx {} def
/Tj {} def

% compound path operators
/CRender {} def

% printing
/_AI3_savepage {} def

% color operands
/_gf null def
/_cf 4 array def
/_if null def
/_of false def
/_fc {} def
/_gs null def
/_cs 4 array def
/_is null def
/_os false def
/_sc {} def
/_i null def
Adobe_IllustratorA_AI3 begin
Adobe_IllustratorA_AI3
	{
	dup xcheck
		{
		bind
		} if
	pop pop
	} forall
end
end
Adobe_IllustratorA_AI3 begin
Adobe_IllustratorA_AI3_vars begin
newpath
} def
/terminate				% - terminate -
{
end
end
} def
% definition operators
/_					% - _ null
null def
/ddef				% key value ddef -
{
Adobe_IllustratorA_AI3_vars 3 1 roll put
} def
/xput				% key value literal xput -
{
dup load dup length exch maxlength eq
	{
	dup dup load dup
	length 2 mul dict copy def
	} if
load begin def end
} def
/npop				% integer npop -
{
	{
	pop
	} repeat
} def
% marking operators
/sw					% ax ay string sw x y 
{
dup length exch stringwidth
exch 5 -1 roll 3 index 1 sub mul add
4 1 roll 3 1 roll 1 sub mul add
} def
/swj				% cx cy fillchar ax ay string swj x y
{
dup 4 1 roll
dup length exch stringwidth 
exch 5 -1 roll 3 index 1 sub mul add
4 1 roll 3 1 roll 1 sub mul add 
6 2 roll /_cnt 0 ddef
{1 index eq {/_cnt _cnt 1 add ddef} if} forall pop
exch _cnt mul exch _cnt mul 2 index add 4 1 roll 2 index add 4 1 roll pop pop
} def
/ss					% ax ay string matrix ss -
{
4 1 roll
	{				% matrix ax ay char 0 0 {proc} -
	2 npop 
	(0) exch 2 copy 0 exch put pop
	gsave
	false charpath currentpoint
	4 index setmatrix
	stroke
	grestore
	moveto
	2 copy rmoveto
	} exch cshow
3 npop
} def
/jss				% cx cy fillchar ax ay string matrix jss -
{
4 1 roll
	{				% cx cy fillchar matrix ax ay char 0 0 {proc} -   
	2 npop 
	(0) exch 2 copy 0 exch put 
	gsave
	_sp eq 
		{
		exch 6 index 6 index 6 index 5 -1 roll widthshow  
		currentpoint
		}
		{
		false charpath currentpoint
		4 index setmatrix stroke
		}ifelse
	grestore
	moveto
	2 copy rmoveto
	} exch cshow
6 npop
} def

% path operators
/sp					% ax ay string sp -
{
	{
	2 npop (0) exch
	2 copy 0 exch put pop
	false charpath
	2 copy rmoveto
	} exch cshow
2 npop
} def
/jsp					% cx cy fillchar ax ay string jsp -
{
	{					% cx cy fillchar ax ay char 0 0 {proc} -
	2 npop 
	(0) exch 2 copy 0 exch put 
	_sp eq 
		{
		exch 5 index 5 index 5 index 5 -1 roll widthshow  
		}
		{
		false charpath
		}ifelse
	2 copy rmoveto
	} exch cshow
5 npop
} def

% path construction operators
/pl				% x y pl x y
{
transform
0.25 sub round 0.25 add exch
0.25 sub round 0.25 add exch
itransform
} def
/setstrokeadjust where
	{
	pop true setstrokeadjust
	/c				% x1 y1 x2 y2 x3 y3 c -
	{
	curveto
	} def
	/C
	/c load def
	/v				% x2 y2 x3 y3 v -
	{
	currentpoint 6 2 roll curveto
	} def
	/V
	/v load def
	/y				% x1 y1 x2 y2 y -
	{
	2 copy curveto
	} def
	/Y
	/y load def
	/l				% x y l -
	{
	lineto
	} def
	/L
	/l load def
	/m				% x y m -
	{
	moveto
	} def
	}
	{%else
	/c
	{
	pl curveto
	} def
	/C
	/c load def
	/v
	{
	currentpoint 6 2 roll pl curveto
	} def
	/V
	/v load def
	/y
	{
	pl 2 copy curveto
	} def
	/Y
	/y load def
	/l
	{
	pl lineto
	} def
	/L
	/l load def
	/m
	{
	pl moveto
	} def
	}ifelse

% graphic state operators
/d					% array phase d -
{
setdash
} def
/cf	{} def			% - cf flatness
/i					% flatness i -
{
dup 0 eq
	{
	pop cf
	} if
setflat
} def
/j					% linejoin j -
{
setlinejoin
} def
/J					% linecap J -
{
setlinecap
} def
/M					% miterlimit M -
{
setmiterlimit
} def
/w					% linewidth w -
{
setlinewidth
} def

% path painting operators
/H					% - H -
{} def
/h					% - h -
{
closepath
} def
/N					% - N -
{
_pola 0 eq 
	{
	_doClip 1 eq {clip /_doClip 0 ddef} if 
	newpath
	} 
	{
	/CRender {N} ddef
	}ifelse
} def
/n					% - n -
{N} def
/F					% - F -
{
_pola 0 eq 
	{
	_doClip 1 eq 
		{
		gsave _pf grestore clip newpath /_lp /none ddef _fc 
		/_doClip 0 ddef
		}
		{
		_pf
		}ifelse
	} 
	{
	/CRender {F} ddef
	}ifelse
} def
/f					% - f -
{
closepath
F
} def
/S					% - S -
{
_pola 0 eq 
	{
	_doClip 1 eq 
		{
		gsave _ps grestore clip newpath /_lp /none ddef _sc 
		/_doClip 0 ddef
		}
		{
		_ps
		}ifelse
	} 
	{
	/CRender {S} ddef
	}ifelse
} def
/s					% - s -
{
closepath
S
} def
/B					% - B -
{
_pola 0 eq 
	{
	_doClip 1 eq 	% F clears _doClip
	gsave F grestore 
		{
		gsave S grestore clip newpath /_lp /none ddef _sc
		/_doClip 0 ddef
		} 
		{
		S
		}ifelse
	}
	{
	/CRender {B} ddef
	}ifelse
} def
/b					% - b -
{
closepath
B
} def
/W					% - W -
{
/_doClip 1 ddef
} def
/*					% - [string] * -
{
count 0 ne 
	{
	dup type (stringtype) eq {pop} if
	} if 
_pola 0 eq {newpath} if
} def

% group operators
/u					% - u -
{} def
/U					% - U -
{} def
/q					% - q -
{
_pola 0 eq {gsave} if
} def
/Q					% - Q -
{
_pola 0 eq {grestore} if
} def
/*u					% - *u -
{
_pola 1 add /_pola exch ddef
} def
/*U					% - *U -
{
_pola 1 sub /_pola exch ddef 
_pola 0 eq {CRender} if
} def
/D					% polarized D -
{pop} def
/*w					% - *w -
{} def
/*W					% - *W -
{} def

% place operators
/`					% matrix llx lly urx ury string ` -
{
/_i save ddef
6 1 roll 4 npop
concat
userdict begin
/showpage {} def
false setoverprint
pop
} def
/~					% - ~ -
{
end
_i restore
} def

% color operators
/O					% flag O -
{
0 ne
/_of exch ddef
/_lp /none ddef
} def
/R					% flag R -
{
0 ne
/_os exch ddef
/_lp /none ddef
} def
/g					% gray g -
{
/_gf exch ddef
/_fc
{ 
_lp /fill ne
	{
	_of setoverprint
	_gf setgray
	/_lp /fill ddef
	} if
} ddef
/_pf
{
_fc
fill
} ddef
/_psf
{
_fc
ashow
} ddef
/_pjsf
{
_fc
awidthshow
} ddef
/_lp /none ddef
} def
/G					% gray G -
{
/_gs exch ddef
/_sc
{
_lp /stroke ne
	{
	_os setoverprint
	_gs setgray
	/_lp /stroke ddef
	} if
} ddef
/_ps
{
_sc
stroke
} ddef
/_pss
{
_sc
ss
} ddef
/_pjss
{
_sc
jss
} ddef
/_lp /none ddef
} def
/k					% cyan magenta yellow black k -
{
_cf astore pop
/_fc
{
_lp /fill ne
	{
	_of setoverprint
	_cf aload pop setcmykcolor
	/_lp /fill ddef
	} if
} ddef
/_pf
{
_fc
fill
} ddef
/_psf
{
_fc
ashow
} ddef
/_pjsf
{
_fc
awidthshow
} ddef
/_lp /none ddef
} def
/K					% cyan magenta yellow black K -
{
_cs astore pop
/_sc
{
_lp /stroke ne
	{
	_os setoverprint
	_cs aload pop setcmykcolor
	/_lp /stroke ddef
	} if
} ddef
/_ps
{
_sc
stroke
} ddef
/_pss
{
_sc
ss
} ddef
/_pjss
{
_sc
jss
} ddef
/_lp /none ddef
} def
/x					% cyan magenta yellow black name gray x -
{
/_gf exch ddef
findcmykcustomcolor
/_if exch ddef
/_fc
{ 
_lp /fill ne
	{
	_of setoverprint
	_if _gf 1 exch sub setcustomcolor
	/_lp /fill ddef
	} if
} ddef
/_pf
{
_fc
fill
} ddef
/_psf
{
_fc
ashow
} ddef
/_pjsf
{
_fc
awidthshow
} ddef
/_lp /none ddef
} def
/X					% cyan magenta yellow black name gray X -
{
/_gs exch ddef
findcmykcustomcolor
/_is exch ddef
/_sc
{
_lp /stroke ne
	{
	_os setoverprint
	_is _gs 1 exch sub setcustomcolor
	/_lp /stroke ddef
	} if
} ddef
/_ps
{
_sc
stroke
} ddef
/_pss
{
_sc
ss
} ddef
/_pjss
{
_sc
jss
} ddef
/_lp /none ddef
} def

% locked object operator
/A					% value A -
{
pop
} def

currentdict readonly pop end
setpacking

% annotate page operator
/annotatepage
{
} def
%%EndResource
%/showpage{}def
/copypage{}def
18 8 translate
[1 0 0 1 0 neg 0 neg] concat
%AI3-Grid.0 18 18 3 0.833333 0.833333 0.833333 3
%%EndProlog
%%BeginSetup
Adobe_cmykcolor /initialize get exec
Adobe_cshow /initialize get exec
Adobe_customcolor /initialize get exec
Adobe_typography_AI3 /initialize get exec
Adobe_IllustratorA_AI3 /initialize get exec
[
39/quotesingle 96/grave 130/quotesinglbase 131/florin 132/quotedblbase
133/ellipsis 134/dagger 135/daggerdbl 136/circumflex 137/perthousand 
138/Scaron 139/guilsinglleft 140/OE 145/quoteleft 146/quoteright 
147/quotedblleft 148/quotedblright 149/bullet 150/endash 151/emdash 
152/tilde 153/trademark 154/scaron 155/guilsinglright 156/oe 157/dotlessi 
159/Ydieresis 164/currency 166/brokenbar 168/dieresis 169/copyright 
170/ordfeminine 172/logicalnot 174/registered 175/macron 176/ring 
177/plusminus 178/twosuperior 179/threesuperior 180/acute 181/mu 
183/periodcentered 184/cedilla 185/onesuperior 186/ordmasculine 
188/onequarter 189/onehalf 190/threequarters 192/Agrave 193/Aacute 
194/Acircumflex 195/Atilde 196/Adieresis 197/Aring 198/AE 199/Ccedilla 
200/Egrave 201/Eacute 202/Ecircumflex 203/Edieresis 204/Igrave 205/Iacute 
206/Icircumflex 207/Idieresis 208/Eth 209/Ntilde 210/Ograve 211/Oacute 
212/Ocircumflex 213/Otilde 214/Odieresis 215/multiply 216/Oslash 
217/Ugrave 218/Uacute 219/Ucircumflex 220/Udieresis 221/Yacute 222/Thorn 
223/germandbls 224/agrave 225/aacute 226/acircumflex 227/atilde 228/adieresis 
229/aring 230/ae 231/ccedilla 232/egrave 233/eacute 234/ecircumflex 
235/edieresis 236/igrave 237/iacute 238/icircumflex 239/idieresis 
240/eth 241/ntilde 242/ograve 243/oacute 244/ocircumflex 245/otilde 
246/odieresis 247/divide 248/oslash 249/ugrave 250/uacute 251/ucircumflex 
252/udieresis 253/yacute 254/thorn 255/ydieresis
TE
%AI3_BeginEncoding: _Times-Roman Times-Roman
[/_Times-Roman/Times-Roman 0 0 1 TZ
%AI3_EndEncoding
%AI3_BeginEncoding: _Times-Italic Times-Italic
[/_Times-Italic/Times-Italic 0 0 1 TZ
%AI3_EndEncoding
/_AI3_savepage save def
%%EndSetup
0 A
u
0 R
0 G
0 i 1 J 1 j 0.25 w 4 M [1 2 ]0 d
%AI3_Note:
0 D
112.3077 634.8376 m
112.3164 114.2958 l
S
1 w []0 d
112.3077 634.8376 m
112.3078 629.1695 l
S
112.3164 114.2958 m
112.3163 119.9639 l
S
0 To
0 -1.3182 1.4362 0 105.6006 645.91 0 Tp
TP
-7 0 Td
0 Tr
0 O
0 g
0 J 0 j
/_Times-Roman 14 Tf
0 Ts
100 Tz
0 Tt
0 TA
0 0 5 TC
100 100 200 TW
0 0 0 Ti
2 Ta
0 Tq
0 0 Tl
0 Tc
0 Tw
(0) Tx 
(\r) TX 
TO
0 R
0 G
165.0152 634.8383 m
165.0153 629.1702 l
S
165.0239 114.2965 m
165.0238 119.9646 l
S
0 To
0 -1.3182 1.4362 0 158.3081 645.9108 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(0.2) Tx 
(\r) TX 
TO
0 R
0 G
217.8664 634.839 m
217.8665 629.171 l
S
217.8751 114.2973 m
217.875 119.9654 l
S
0 To
0 -1.3182 1.4362 0 211.1593 645.9115 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(0.4) Tx 
(\r) TX 
TO
0 R
0 G
270.5739 634.8398 m
270.574 629.1717 l
S
270.5826 114.298 m
270.5825 119.9661 l
S
0 To
0 -1.3182 1.4362 0 263.8668 645.9122 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(0.6) Tx 
(\r) TX 
TO
0 R
0 G
323.2815 634.8405 m
323.2816 629.1724 l
S
323.2901 114.2987 m
323.29 119.9668 l
S
0 To
0 -1.3182 1.4362 0 316.5744 645.913 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(0.8) Tx 
(\r) TX 
TO
0 R
0 G
375.989 634.8413 m
375.9891 629.1732 l
S
375.9976 114.2995 m
375.9976 119.9676 l
S
0 To
0 -1.3182 1.4362 0 369.2819 645.9137 0 Tp
TP
-7 0 Td
0 Tr
0 O
0 g
(1) Tx 
(\r) TX 
TO
0 R
0 G
428.6965 634.842 m
428.6966 629.1739 l
S
428.7052 114.3002 m
428.7051 119.9683 l
S
0 To
0 -1.3182 1.4362 0 421.9894 645.9145 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(1.2) Tx 
(\r) TX 
TO
0 R
0 G
481.5477 634.8427 m
481.5478 629.1747 l
S
481.5563 114.301 m
481.5562 119.9691 l
S
0 To
0 -1.3182 1.4362 0 474.8406 645.9152 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(1.4) Tx 
(\r) TX 
TO
0 R
0 G
534.2552 634.8435 m
534.2553 629.1754 l
S
534.2639 114.3017 m
534.2638 119.9698 l
S
0 To
0 -1.3182 1.4362 0 527.5481 645.916 0 Tp
TP
-17.5 0 Td
0 Tr
0 O
0 g
(1.6) Tx 
(\r) TX 
TO
0 R
0 G
112.3077 634.8376 m
118.4833 634.8377 l
S
534.2552 634.8435 m
528.0796 634.8434 l
S
0 To
0 -1.3182 1.4362 0 85.4944 634.8372 0 Tp
TP
-8.75 0 Td
0 Tr
0 O
0 g
1 Ta
(0.2) Tx 
(\r) TX 
TO
0 R
0 G
112.3091 549.1571 m
118.4847 549.1572 l
S
534.2566 549.163 m
528.0811 549.1629 l
S
0 To
0 -1.3182 1.4362 0 85.4958 549.1567 0 Tp
TP
-12.25 0 Td
0 Tr
0 O
0 g
(0.25) Tx 
(\r) TX 
TO
0 R
0 G
112.3106 463.6084 m
118.4861 463.6085 l
S
534.2581 463.6144 m
528.0825 463.6143 l
S
0 To
0 -1.3182 1.4362 0 85.4972 463.6081 0 Tp
TP
-8.75 0 Td
0 Tr
0 O
0 g
(0.3) Tx 
(\r) TX 
TO
0 R
0 G
112.312 377.928 m
118.4875 377.9281 l
S
534.2595 377.9339 m
528.0839 377.9338 l
S
0 To
0 -1.3182 1.4362 0 85.4987 377.9276 0 Tp
TP
-12.25 0 Td
0 Tr
0 O
0 g
(0.35) Tx 
(\r) TX 
TO
0 R
0 G
112.3134 292.3793 m
118.489 292.3794 l
S
534.2609 292.3852 m
528.0854 292.3852 l
S
0 To
0 -1.3182 1.4362 0 85.5001 292.379 0 Tp
TP
-8.75 0 Td
0 Tr
0 O
0 g
(0.4) Tx 
(\r) TX 
TO
0 R
0 G
112.3148 206.6989 m
118.4904 206.699 l
S
534.2623 206.7048 m
528.0868 206.7047 l
S
0 To
0 -1.3182 1.4362 0 85.5015 206.6985 0 Tp
TP
-12.25 0 Td
0 Tr
0 O
0 g
(0.45) Tx 
(\r) TX 
TO
0 R
0 G
112.3163 121.1502 m
118.4918 121.1503 l
S
534.2637 121.1561 m
528.0882 121.156 l
S
0 To
0 -1.3182 1.4362 0 85.5029 121.1499 0 Tp
TP
-8.75 0 Td
0 Tr
0 O
0 g
(0.5) Tx 
(\r) TX 
TO
0 R
0 G
112.3077 634.8376 m
112.3164 114.2958 l
534.2639 114.3017 l
534.2552 634.8435 l
112.3077 634.8376 l
S
0 To
1.4362 0 0 1.3182 323.2798 695.047 0 Tp
TP
-28.3691 0 Td
0 Tr
0 O
0 g
/_Times-Italic 14 Tf
99.9999 Tz
(H) Tx 
/_Times-Roman 14 Tf
100 Tz
(  \(Tesla\)) Tx 
(\r) TX 
TO
0 To
0 -1.3182 1.4362 0 45.6655 374.6319 0 Tp
TP
-15.3535 0 Td
0 Tr
/_Times-Italic 14 Tf
99.9999 Tz
(T) Tx 
/_Times-Roman 14 Tf
100 Tz
( \(K\)) Tx 
(\r) TX 
TO
0 To
1.3182 0 0 1.4362 346.6927 42.9826 0 Tp
TP
-99.345 0 Td
0 Tr
(K. A. Park and Robert Joynt, Fig. 1) Tx 
(\r) TX 
TO
0 R
0 G
0.5 w [4 2 ]0 d
112.3143 241.2347 m
112.3143 241.2347 l
117.6281 240.9711 l
122.942 240.9712 l
128.2558 240.9713 l
133.5696 241.1032 l
138.8835 241.3669 l
144.3409 241.7624 l
149.6547 242.2897 l
154.9686 242.9489 l
160.2824 243.8717 l
165.5962 244.7945 l
170.91 245.8491 l
176.2238 247.1673 l
181.5377 248.4856 l
186.8515 250.0674 l
192.1653 251.7811 l
197.6227 253.4948 l
202.9365 255.4721 l
208.2503 257.5812 l
213.5641 259.8222 l
218.8779 262.1949 l
224.1917 264.6995 l
229.5055 267.3359 l
234.8193 270.1041 l
240.1331 273.136 l
245.4469 276.1678 l
250.7607 279.4633 l
256.218 282.8906 l
261.5319 286.5815 l
266.8456 290.2724 l
272.1594 294.227 l
277.4732 298.3134 l
282.7869 302.5316 l
288.1007 307.0134 l
293.4144 311.7589 l
298.7282 316.5043 l
304.042 321.6452 l
309.4993 326.9179 l
314.8131 332.4543 l
320.1268 338.2542 l
325.4406 344.3179 l
330.7543 350.5133 l
336.068 357.1042 l
341.3817 364.0905 l
346.6954 371.2086 l
352.0092 378.7222 l
357.3229 386.3676 l
362.7802 394.4085 l
368.0939 402.8448 l
373.4076 411.4129 l
378.7213 420.2447 l
384.035 429.3401 l
389.3487 438.6991 l
394.6623 448.3217 l
399.976 458.0762 l
405.2897 468.0943 l
410.6033 478.2442 l
415.917 488.6578 l
421.3743 499.2031 l
426.688 509.8803 l
432.0016 520.8211 l
437.3153 531.7619 l
442.6289 543.0982 l
447.9426 554.4344 l
453.2562 565.9025 l
458.5699 577.6342 l
463.8835 589.4978 l
469.1972 601.4931 l
474.6544 613.6203 l
479.968 625.8792 l
483.7019 634.8428 l
S
[]0 d
112.3163 121.1502 m
112.3163 121.1502 l
117.63 123.3912 l
122.9439 125.8958 l
128.2577 128.4003 l
133.5715 131.0367 l
138.8852 133.9367 l
144.3426 136.8368 l
149.6564 139.8686 l
154.9702 143.1641 l
160.284 146.4596 l
165.5978 149.8869 l
170.9116 153.5778 l
176.2254 157.2687 l
181.5391 161.0915 l
186.8529 165.1779 l
192.1667 169.2642 l
197.624 173.4824 l
202.9378 177.8324 l
208.2516 182.446 l
213.5653 187.0597 l
218.8791 191.8052 l
224.1929 196.6824 l
229.5066 201.6915 l
234.8204 206.8324 l
240.1341 212.1051 l
245.4479 217.5097 l
250.7616 223.046 l
256.2189 228.7142 l
261.5327 234.3824 l
266.8465 240.3141 l
272.1602 246.246 l
277.4739 252.4414 l
282.7877 258.6368 l
288.1014 264.9641 l
293.4151 271.4231 l
298.7288 278.014 l
304.0426 284.6049 l
309.4999 291.3276 l
314.8136 298.1821 l
320.1273 305.1684 l
325.4411 312.1548 l
330.7548 319.2729 l
336.0685 326.391 l
341.3822 333.641 l
346.6959 340.8909 l
352.0097 348.2727 l
357.3234 355.7863 l
362.7807 363.1681 l
368.0944 370.8135 l
373.4082 378.4589 l
378.7219 386.2361 l
384.0356 394.0134 l
389.3493 401.9224 l
394.663 409.9633 l
399.9767 418.0041 l
405.2904 426.1768 l
410.6041 434.6131 l
415.9178 443.0494 l
421.3751 451.4857 l
426.6888 460.1856 l
432.0025 469.0174 l
437.3162 477.8491 l
442.6299 486.8127 l
447.9435 496.0399 l
453.2572 505.2671 l
458.5709 514.6261 l
463.8846 524.117 l
469.1983 533.7396 l
474.6556 543.6259 l
479.9692 553.5122 l
485.2829 563.5303 l
490.5966 573.6802 l
495.9103 583.9619 l
501.2239 594.2437 l
506.5376 604.789 l
511.8512 615.4662 l
517.1649 626.2752 l
521.3296 634.8433 l
S
512.1392 569.726 m
509.1233 566.9578 l
512.1393 564.1897 l
515.1552 566.9579 l
512.1392 569.726 l
S
512.1393 566.9579 m
512.1393 566.9579 l
S
465.3213 494.722 m
462.3053 491.9538 l
465.3213 489.1857 l
468.3373 491.9539 l
465.3213 494.722 l
S
465.3213 491.9539 m
465.3213 491.9539 l
S
468.4809 491.4266 m
465.465 488.6585 l
468.481 485.8903 l
471.4969 488.6585 l
468.4809 491.4266 l
S
468.4809 488.6585 m
468.4809 488.6585 l
S
441.9122 463.0858 m
438.8963 460.3176 l
441.9123 457.5495 l
444.9282 460.3177 l
441.9122 463.0858 l
S
441.9122 460.3177 m
441.9122 460.3177 l
S
428.1251 454.6494 m
425.1091 451.8812 l
428.1251 449.1131 l
431.141 451.8813 l
428.1251 454.6494 l
S
428.1251 451.8813 m
428.1251 451.8813 l
S
386.6206 401.2633 m
383.6047 398.4951 l
386.6206 395.727 l
389.6366 398.4952 l
386.6206 401.2633 l
S
386.6206 398.4951 m
386.6206 398.4951 l
S
393.0834 399.6816 m
390.0675 396.9134 l
393.0834 394.1453 l
396.0994 396.9135 l
393.0834 399.6816 l
S
393.0834 396.9134 m
393.0834 396.9134 l
S
383.4611 391.377 m
380.4452 388.6089 l
383.4612 385.8407 l
386.4772 388.6089 l
383.4611 391.377 l
S
383.4612 388.6089 m
383.4612 388.6089 l
S
374.9879 382.9407 m
371.972 380.1725 l
374.988 377.4044 l
378.0039 380.1726 l
374.9879 382.9407 l
S
374.9879 380.1725 m
374.9879 380.1725 l
S
366.5146 372.9225 m
363.4987 370.1544 l
366.5147 367.3863 l
369.5306 370.1545 l
366.5146 372.9225 l
S
366.5147 370.1544 m
366.5147 370.1544 l
S
360.0519 367.9134 m
357.036 365.1453 l
360.052 362.3771 l
363.0679 365.1453 l
360.0519 367.9134 l
S
360.052 365.1453 m
360.052 365.1453 l
S
350.5733 357.8953 m
347.5574 355.1271 l
350.5735 352.359 l
353.5894 355.1272 l
350.5733 357.8953 l
S
350.5734 355.1271 m
350.5734 355.1271 l
S
343.1053 351.3044 m
340.0895 348.5362 l
343.1054 345.7681 l
346.1214 348.5363 l
343.1053 351.3044 l
S
343.1054 348.5362 m
343.1054 348.5362 l
S
338.797 341.2863 m
335.7811 338.5181 l
338.7971 335.75 l
341.813 338.5182 l
338.797 341.2863 l
S
338.797 338.5182 m
338.797 338.5182 l
S
325.0101 322.9637 m
321.9941 320.1955 l
325.0102 317.4274 l
328.0261 320.1956 l
325.0101 322.9637 l
S
325.0101 320.1955 m
325.0101 320.1955 l
S
318.5474 314.6591 m
315.5315 311.891 l
318.5475 309.1229 l
321.5634 311.891 l
318.5474 314.6591 l
S
318.5475 311.891 m
318.5475 311.891 l
S
298.4414 291.1956 m
295.4255 288.4274 l
298.4415 285.6593 l
301.4574 288.4275 l
298.4414 291.1956 l
S
298.4414 288.4275 m
298.4414 288.4275 l
S
270.7238 259.5594 m
267.7079 256.7912 l
270.7239 254.0231 l
273.7398 256.7913 l
270.7238 259.5594 l
S
270.7238 256.7912 m
270.7238 256.7912 l
S
267.5643 251.2549 m
264.5484 248.4867 l
267.5645 245.7186 l
270.5803 248.4868 l
267.5643 251.2549 l
S
267.5644 248.4868 m
267.5644 248.4868 l
S
260.0963 246.2458 m
257.0804 243.4776 l
260.0964 240.7095 l
263.1123 243.4777 l
260.0963 246.2458 l
S
260.0964 243.4776 m
260.0964 243.4776 l
S
245.304 229.5049 m
242.2881 226.7368 l
245.3041 223.9686 l
248.32 226.7368 l
245.304 229.5049 l
S
245.3041 226.7368 m
245.3041 226.7368 l
S
218.5916 204.4595 m
215.5757 201.6913 l
218.5917 198.9232 l
221.6077 201.6914 l
218.5916 204.4595 l
S
218.5917 201.6913 m
218.5917 201.6913 l
S
192.023 174.5369 m
189.0071 171.7687 l
192.0231 169.0006 l
195.039 171.7688 l
192.023 174.5369 l
S
192.023 171.7687 m
192.023 171.7687 l
S
185.7038 172.8232 m
182.6879 170.055 l
185.7039 167.2869 l
188.7198 170.0551 l
185.7038 172.8232 l
S
185.7039 170.055 m
185.7039 170.055 l
S
165.4541 154.5004 m
162.4382 151.7322 l
165.4542 148.9642 l
168.4701 151.7323 l
165.4541 154.5004 l
S
165.4541 151.7323 m
165.4541 151.7323 l
S
138.8852 136.1776 m
135.8693 133.4095 l
138.8853 130.6414 l
141.9012 133.4095 l
138.8852 136.1776 l
S
138.8853 133.4095 m
138.8853 133.4095 l
S
112.3162 127.741 m
109.3002 124.9729 l
112.3162 122.2047 l
115.3322 124.973 l
112.3162 127.741 l
S
112.3162 124.9729 m
112.3162 124.9729 l
S
428.1223 621.5286 m
425.1064 618.7604 l
428.1224 615.9923 l
431.1383 618.7605 l
428.1223 621.5286 l
S
428.1223 618.7604 m
428.1223 618.7604 l
S
407.8731 571.4382 m
404.8572 568.67 l
407.8732 565.9019 l
410.8891 568.6701 l
407.8731 571.4382 l
S
407.8731 568.67 m
407.8731 568.67 l
S
415.3412 568.1429 m
412.3253 565.3747 l
415.3413 562.6066 l
418.3572 565.3748 l
415.3412 568.1429 l
S
415.3413 565.3747 m
415.3413 565.3747 l
S
394.0871 494.721 m
391.0712 491.9528 l
394.0872 489.1847 l
397.1031 491.9529 l
394.0871 494.721 l
S
394.0871 491.9529 m
394.0871 491.9529 l
S
401.5553 489.7121 m
398.5394 486.9439 l
401.5554 484.1758 l
404.5713 486.944 l
401.5553 489.7121 l
S
401.5553 486.944 m
401.5553 486.944 l
S
367.5194 402.9766 m
364.5035 400.2084 l
367.5195 397.4403 l
370.5354 400.2085 l
367.5194 402.9766 l
S
367.5195 400.2085 m
367.5195 400.2085 l
S
323.8606 353.0177 m
320.8447 350.2495 l
323.8607 347.4814 l
326.8766 350.2496 l
323.8606 353.0177 l
S
323.8607 350.2496 m
323.8607 350.2496 l
S
297.2918 329.5541 m
294.2759 326.7859 l
297.2919 324.0178 l
300.3078 326.786 l
297.2918 329.5541 l
S
297.2919 326.7859 m
297.2919 326.7859 l
S
288.8185 321.2495 m
285.8026 318.4813 l
288.8186 315.7133 l
291.8345 318.4814 l
288.8185 321.2495 l
S
288.8186 318.4814 m
288.8186 318.4814 l
S
271.8719 312.9449 m
268.8559 310.1767 l
271.8719 307.4086 l
274.8878 310.1768 l
271.8719 312.9449 l
S
271.8719 310.1768 m
271.8719 310.1768 l
S
244.1539 301.2129 m
241.138 298.4447 l
244.154 295.6766 l
247.1699 298.4448 l
244.1539 301.2129 l
S
244.154 298.4447 m
244.154 298.4447 l
S
232.5211 287.8993 m
229.5052 285.1311 l
232.5212 282.363 l
235.5372 285.1312 l
232.5211 287.8993 l
S
232.5212 285.1311 m
232.5212 285.1311 l
S
218.5904 279.5946 m
215.5745 276.8265 l
218.5905 274.0584 l
221.6064 276.8266 l
218.5904 279.5946 l
S
218.5904 276.8265 m
218.5904 276.8265 l
S
165.4525 247.8262 m
162.4366 245.0581 l
165.4526 242.29 l
168.4686 245.0581 l
165.4525 247.8262 l
S
165.4526 245.0581 m
165.4526 245.0581 l
S
138.8836 234.5124 m
135.8677 231.7443 l
138.8837 228.9762 l
141.8996 231.7444 l
138.8836 234.5124 l
S
138.8836 231.7443 m
138.8836 231.7443 l
S
112.3145 229.503 m
109.2986 226.7349 l
112.3146 223.9668 l
115.3305 226.735 l
112.3145 229.503 l
S
112.3145 226.7349 m
112.3145 226.7349 l
S
U
%%PageTrailer
_AI3_savepage restore
gsave annotatepage grestore
%%Trailer
Adobe_IllustratorA_AI3 /terminate get exec
Adobe_typography_AI3 /terminate get exec
Adobe_customcolor /terminate get exec
Adobe_cshow /terminate get exec
Adobe_cmykcolor /terminate get exec
Adobe_packedarray /terminate get exec
%%EndDocument
1 #C
statusdict begin /manualfeed false store end
EJ RS
%%PageTrailer
%%PageResources: 
2394 3231 0 0 CB
%%Trailer
SVDoc restore
end
%%Pages: 1
%%DocumentSuppliedResources: procset Win35Dict 3 1

%%DocumentNeededResources: 
%%EOF

